Strong Dependence of Type Ia Supernova Standardization on the Local Specific Star Formation Rate

As part of an on-going effort to identify, understand and correct for astrophysics biases in the standardization of Type Ia supernovae (SNIa) for cosmology, we have statistically classified a large sample of nearby SNeIa into those located in predominantly younger or older environments. This classification is based on the specific star formation rate measured within a projected distance of 1kpc from each SN location (LsSFR). This is an important refinement compared to using the local star formation rate directly as it provides a normalization for relative numbers of available SN progenitors and is more robust against extinction by dust. We find that the SNeIa in predominantly younger environments are DY=0.163\pm0.029 mag (5.7 sigma) fainter than those in predominantly older environments after conventional light-curve standardization. This is the strongest standardized SN Ia brightness systematic connected to host-galaxy environment measured to date. The well-established step in standardized brightnesses between SNeIa in hosts with lower or higher total stellar masses is smaller at DM=0.119\pm0.032 mag (4.5 sigma), for the same set of SNeIa. When fit simultaneously, the environment age offset remains very significant, with DY=0.129\pm0.032 mag (4.0 sigma), while the global stellar mass step is reduced to DM=0.064\pm0.029 mag (2.2 sigma). Thus, approximately 70% of the variance from the stellar mass step is due to an underlying dependence on environment-based progenitor age. Standardization using only the SNeIa in younger environments reduces the total dispersion from 0.142\pm0.008 mag to 0.120\pm0.010 mag. We show that as environment ages evolve with redshift a strong bias on measurement of the dark energy equation of state parameters can develop. Fortunately, data to measure and correct for this effect is likely to be available for many next-generation experiments. [abstract shorten]

==> datatable.tex <==
\begin{landscape}
\begin{longtable}{l|ccccccccccc}

%\centering
\caption{Data for the \nSNe\ SNe~Ia used in this analysis.} \label{tab:datalong}\\
%\footnotesize{
%\renewcommand{\arraystretch}{1.3}
%\setlength{\tabcolsep}{3pt}


\hline\hline%\\[-0.8em]
{SN Name} & {$\Delta\,m_B^{corr}$} & {$z_{CMB}$} & {$c$} & {$x_1$} & {Local Mass} & {Local SFR} &
{Local sSFR} & {Global Mass} & {\PY} & {\PM} & {Refs}\\[-0.5em]
                & \small{$\mathrm{mag}$} & & & & \small{$\log(\mathrm{M_*/M_\odot})$} &
\small{$\log(\mathrm{M_*\, yr^{-1}\,kpc^{-2}})$} &
                                            \small{$\log(\mathrm{yr^{-1}\,kpc^{-2}})$}&
                                                                                \small{$\log(\mathrm{M_*/M_\odot})$}
                         & \small{\%} & \small{\%} & \\[0.15em]
\hline\\[-0.8em]

\endfirsthead

\caption{continued.}\\

\hline\hline%\\[-0.8em]
{SN Name} & {$\Delta\,m_B^{corr}$} & {$z_{CMB}$} &{$c$} & {$x_1$} & {Local Mass} & {Local SFR} &
{Local sSFR} & {Global Mass} & {\PY} & {\PM} & {Notes}\\[-0.5em]
                & \small{$\mathrm{mag}$} & & & & \small{$\log(\mathrm{M_*/M_\odot})$} &
\small{$\log(\mathrm{M_*\, yr^{-1}\,kpc^{-2}})$} &
                                            \small{$\log(\mathrm{yr^{-1}\,kpc^{-2}})$}&
                                                                                \small{$\log(\mathrm{M_*/M_\odot})$}
                         & \small{\%} & \small{\%} & \\[0.15em]
\hline\\[-0.8em]

\endhead

%\hline\\[-0.8em]
\endfoot

\endlastfoot
SNF20050624-000 & $-0.23\pm{0.13}$ & $0.0671$ & $-0.07\pm{0.03}$ & $+0.20\pm{0.55}$ & $7.33^{+0.38}_{-0.51}$ &$-4.74^{+0.50}_{-0.60}$&$-12.0^{+0.7}_{-0.7}$& $10.73^{+0.10}_{-0.10}$ & 4 & 100 & -- \\[0.20em]
SNF20050728-000 & $-0.19\pm{0.13}$ & $0.0419$ & $-0.03\pm{0.03}$ & $+0.77\pm{0.24}$ & $8.00^{+0.11}_{-0.11}$ &$-2.39^{+0.01}_{-0.01}$&$-10.4^{+0.1}_{-0.1}$& $8.53^{+0.10}_{-0.10}$ & 100 & 0 & -- \\[0.20em]
SNF20050728-006 & $-0.03\pm{0.12}$ & $0.0581$ & $+0.09\pm{0.03}$ & $+0.19\pm{0.24}$ & $7.83^{+0.21}_{-0.22}$ &$-3.14^{+0.06}_{-0.06}$&$-11.0^{+0.2}_{-0.2}$& $10.00^{+0.10}_{-0.10}$ & 25 & 50 & -- \\[0.20em]
SNF20050821-007 & $-0.06\pm{0.13}$ & $0.0582$ & $-0.05\pm{0.03}$ & $+0.11\pm{0.32}$ & $7.84^{+0.14}_{-0.14}$ &$-2.46^{+0.02}_{-0.02}$&$-10.3^{+0.1}_{-0.1}$& $8.92^{+0.10}_{-0.10}$ & 99 & 0 & -- \\[0.20em]
SNF20050829-003 & $+0.22\pm{0.14}$ & $0.0440$ & $+0.03\pm{0.04}$ & $-1.44\pm{0.37}$ & $7.61^{+0.21}_{-0.20}$ &$-3.07^{+0.06}_{-0.06}$&$-10.7^{+0.2}_{-0.2}$& $9.90^{+0.10}_{-0.10}$ & 72 & 14 & -- \\[0.20em]
SNF20050927-005 & $+0.25\pm{0.13}$ & $0.0396$ & $+0.02\pm{0.03}$ & $+0.67\pm{0.28}$ & $8.50^{+0.10}_{-0.10}$ &$-1.75^{+0.01}_{-0.01}$&$-10.2^{+0.1}_{-0.1}$& $9.42^{+0.10}_{-0.10}$ & 100 & 0 & -- \\[0.20em]
SNF20051003-004 & $+0.05\pm{0.13}$ & $0.0337$ & $-0.09\pm{0.03}$ & $+1.06\pm{0.15}$ & $8.65^{+0.10}_{-0.10}$ &$-1.88^{+0.01}_{-0.01}$&$-10.5^{+0.1}_{-0.1}$& $9.14^{+0.10}_{-0.10}$ & 99 & 0 & -- \\[0.20em]
SNF20060511-014 & $-0.07\pm{0.14}$ & $0.0467$ & $-0.03\pm{0.03}$ & $-0.65\pm{0.17}$ & $7.55^{+0.25}_{-0.27}$ &$-3.20^{+0.10}_{-0.13}$&$-10.8^{+0.3}_{-0.3}$& $10.20^{+0.10}_{-0.10}$ & 59 & 97 & -- \\[0.20em]
SNF20060512-001 & $-0.06\pm{0.13}$ & $0.0389$ & $+0.02\pm{0.03}$ & $+0.71\pm{0.13}$ & $8.73^{+0.10}_{-0.10}$ &$-1.68^{+0.01}_{-0.01}$&$-10.4^{+0.1}_{-0.1}$& $9.32^{+0.10}_{-0.10}$ & 100 & 0 & -- \\[0.20em]
SNF20060512-002 & $-0.45\pm{0.12}$ & $0.0509$ & $+0.05\pm{0.03}$ & $-0.92\pm{0.19}$ & $9.80^{+0.10}_{-0.10}$ &$-2.00^{+0.01}_{-0.01}$&$-11.8^{+0.1}_{-0.1}$& $10.72^{+0.10}_{-0.10}$ & 0 & 100 & -- \\[0.20em]
SNF20060521-001 & $-0.03\pm{0.13}$ & $0.0679$ & $-0.05\pm{0.03}$ & $-1.15\pm{0.23}$ & $9.22^{+0.10}_{-0.10}$ &$-4.14^{+0.44}_{-0.77}$&$-13.4^{+0.5}_{-0.7}$& $9.88^{+0.10}_{-0.10}$ & 0 & 10 & -- \\[0.20em]
SNF20060521-008 & $-0.27\pm{0.14}$ & $0.0562$ & $+0.09\pm{0.03}$ & $-1.36\pm{0.20}$ & $7.41^{+0.25}_{-0.27}$ &$-3.49^{+0.13}_{-0.22}$&$-10.9^{+0.3}_{-0.4}$& $11.05^{+0.10}_{-0.10}$ & 37 & 100 & -- \\[0.20em]
SNF20060526-003 & $+0.01\pm{0.12}$ & $0.0788$ & $-0.03\pm{0.03}$ & $+0.30\pm{0.14}$ & $7.29^{+0.33}_{-0.42}$ &$-3.08^{+0.07}_{-0.09}$&$-10.4^{+0.4}_{-0.3}$& $10.52^{+0.10}_{-0.10}$ & 90 & 100 & -- \\[0.20em]
SNF20060530-003 & $-0.04\pm{0.12}$ & $0.0572$ & $-0.05\pm{0.03}$ & $+1.06\pm{0.16}$ & $7.96^{+0.13}_{-0.12}$ &$-2.28^{+0.01}_{-0.01}$&$-10.2^{+0.1}_{-0.1}$& $10.14^{+0.10}_{-0.10}$ & 100 & 91 & -- \\[0.20em]
SNF20060609-002 & $-0.07\pm{0.13}$ & $0.0399$ & $+0.20\pm{0.03}$ & $+0.06\pm{0.13}$ & $9.05^{+0.10}_{-0.10}$ &$-1.74^{+0.01}_{-0.01}$&$-10.8^{+0.1}_{-0.1}$& $10.47^{+0.10}_{-0.10}$ & 59 & 100 & -- \\[0.20em]
SNF20060618-014 & $+0.04\pm{0.12}$ & $0.0645$ & $-0.02\pm{0.03}$ & $+0.97\pm{0.16}$ & $8.04^{+0.13}_{-0.12}$ &$-2.47^{+0.02}_{-0.02}$&$-10.5^{+0.1}_{-0.1}$& $8.79^{+0.11}_{-0.10}$ & 99 & 0 & -- \\[0.20em]
SNF20060621-012 & $+0.29\pm{0.12}$ & $0.0618$ & $-0.10\pm{0.03}$ & $-1.03\pm{0.18}$ & $8.35^{+0.12}_{-0.11}$ &$-2.39^{+0.01}_{-0.01}$&$-10.7^{+0.1}_{-0.1}$& $9.19^{+0.10}_{-0.10}$ & 77 & 0 & -- \\[0.20em]
SNF20060621-015 & $-0.02\pm{0.12}$ & $0.0544$ & $-0.09\pm{0.03}$ & $+0.51\pm{0.20}$ & $7.58^{+0.13}_{-0.13}$ &$-2.12^{+0.01}_{-0.01}$&$-9.7^{+0.1}_{-0.1}$& $9.22^{+0.10}_{-0.10}$ & 100 & 0 & -- \\[0.20em]
SNF20060624-019 & $-0.24\pm{0.12}$ & $0.0741$ & $+0.43\pm{0.03}$ & $+0.88\pm{0.19}$ & $8.58^{+0.12}_{-0.11}$ &$-2.31^{+0.02}_{-0.02}$&$-10.9^{+0.1}_{-0.1}$& $10.27^{+0.10}_{-0.10}$ & 27 & 99 & -- \\[0.20em]
SNF20060907-000 & $+0.12\pm{0.12}$ & $0.0564$ & $-0.13\pm{0.03}$ & $+0.08\pm{0.16}$ & $9.12^{+0.10}_{-0.10}$ &$-1.37^{+0.01}_{-0.01}$&$-10.5^{+0.1}_{-0.1}$& $9.64^{+0.10}_{-0.10}$ & 99 & 0 & -- \\[0.20em]
SNF20060912-000 & $-0.28\pm{0.12}$ & $0.0723$ & $+0.10\pm{0.03}$ & $+0.27\pm{0.20}$ & $8.09^{+0.13}_{-0.14}$ &$-2.26^{+0.01}_{-0.01}$&$-10.3^{+0.1}_{-0.1}$& $10.69^{+0.10}_{-0.10}$ & 99 & 100 & -- \\[0.20em]
SNF20060912-004 & $-0.04\pm{0.12}$ & $0.0769$ & $-0.04\pm{0.03}$ & $+0.21\pm{0.37}$ & $7.85^{+0.16}_{-0.17}$ &$-2.84^{+0.04}_{-0.04}$&$-10.7^{+0.2}_{-0.2}$& $10.79^{+0.10}_{-0.10}$ & 77 & 100 & -- \\[0.20em]
SNF20060916-002 & $+0.15\pm{0.13}$ & $0.0716$ & $-0.06\pm{0.03}$ & $+1.49\pm{0.25}$ & $7.82^{+0.15}_{-0.14}$ &$-2.93^{+0.03}_{-0.03}$&$-10.8^{+0.1}_{-0.1}$& $8.95^{+0.10}_{-0.10}$ & 67 & 0 & -- \\[0.20em]
SNF20061011-005 & $+0.06\pm{0.16}$ & $0.0226$ & $-0.14\pm{0.03}$ & $+0.72\pm{0.21}$ & $7.69^{+0.10}_{-0.10}$ &$-2.62^{+0.01}_{-0.01}$&$-10.3^{+0.1}_{-0.1}$& $8.61^{+0.10}_{-0.10}$ & 100 & 0 & -- \\[0.20em]
SNF20061020-000 & $-0.05\pm{0.13}$ & $0.0379$ & $+0.00\pm{0.03}$ & $-1.74\pm{0.17}$ & $8.45^{+0.10}_{-0.10}$ &$-4.63^{+0.33}_{-0.49}$&$-13.1^{+0.3}_{-0.5}$& $10.19^{+0.10}_{-0.10}$ & 0 & 97 & -- \\[0.20em]
SNF20061021-003 & $-0.06\pm{0.12}$ & $0.0615$ & $+0.05\pm{0.03}$ & $+0.27\pm{0.17}$ & $8.42^{+0.12}_{-0.12}$ &$-3.56^{+0.14}_{-0.22}$&$-12.0^{+0.2}_{-0.2}$& $11.07^{+0.10}_{-0.10}$ & 0 & 100 & -- \\[0.20em]
SNF20061022-005 & $-0.09\pm{0.12}$ & $0.0779$ & $+0.06\pm{0.03}$ & $+1.15\pm{0.29}$ & $8.74^{+0.11}_{-0.12}$ &$-2.21^{+0.01}_{-0.01}$&$-10.9^{+0.1}_{-0.1}$& $10.35^{+0.10}_{-0.10}$ & 12 & 100 & -- \\[0.20em]
SNF20061022-014 & $-0.29\pm{0.14}$ & $0.0398$ & $+0.56\pm{0.03}$ & $-2.18\pm{0.33}$ & $8.98^{+0.10}_{-0.10}$ &$-2.42^{+0.01}_{-0.01}$&$-11.4^{+0.1}_{-0.1}$& $10.67^{+0.10}_{-0.10}$ & 0 & 100 & -- \\[0.20em]
SNF20061024-000 & $+0.17\pm{0.12}$ & $0.0559$ & $-0.03\pm{0.03}$ & $-0.90\pm{0.12}$ & $8.20^{+0.13}_{-0.13}$ &$-3.58^{+0.15}_{-0.25}$&$-11.8^{+0.2}_{-0.3}$& $10.63^{+0.10}_{-0.10}$ & 0 & 100 & -- \\[0.20em]
SNF20061030-010 & $+0.03\pm{0.14}$ & $0.0278$ & $+0.13\pm{0.03}$ & $+0.26\pm{0.21}$ & $8.77^{+0.10}_{-0.10}$ &$-1.60^{+0.01}_{-0.01}$&$-10.4^{+0.1}_{-0.1}$& $9.50^{+0.10}_{-0.10}$ & 100 & 0 & -- \\[0.20em]
SNF20061111-002 & $+0.06\pm{0.12}$ & $0.0677$ & $-0.01\pm{0.03}$ & $+0.37\pm{0.20}$ & $7.35^{+0.32}_{-0.42}$ &$-2.51^{+0.02}_{-0.02}$&$-9.8^{+0.4}_{-0.3}$& $8.87^{+0.10}_{-0.11}$ & 99 & 0 & -- \\[0.20em]
SNF20070330-024 & $-0.23\pm{0.12}$ & $0.0417$ & $-0.09\pm{0.03}$ & $+0.46\pm{0.18}$ & $8.82^{+0.10}_{-0.10}$ &$-2.75^{+0.03}_{-0.04}$&$-11.6^{+0.1}_{-0.1}$& $11.02^{+0.10}_{-0.10}$ & 0 & 100 & -- \\[0.20em]
SNF20070331-014 & $-0.04\pm{0.12}$ & $0.0680$ & $-0.00\pm{0.03}$ & $-0.66\pm{0.16}$ & $7.08^{+0.34}_{-0.41}$ &$-3.79^{+0.30}_{-0.50}$&$-10.9^{+0.5}_{-0.6}$& $11.10^{+0.10}_{-0.10}$ & 43 & 100 & -- \\[0.20em]
SNF20070403-000 & $+0.13\pm{0.13}$ & $0.0499$ & $+0.08\pm{0.03}$ & $-2.12\pm{0.17}$ & $8.01^{+0.12}_{-0.12}$ &$-2.96^{+0.04}_{-0.05}$&$-11.0^{+0.1}_{-0.1}$& $9.92^{+0.10}_{-0.10}$ & 11 & 19 & -- \\[0.20em]
SNF20070424-003 & $+0.15\pm{0.12}$ & $0.0682$ & $-0.03\pm{0.03}$ & $+0.35\pm{0.10}$ & $7.45^{+0.21}_{-0.22}$ &$-3.11^{+0.06}_{-0.07}$&$-10.6^{+0.2}_{-0.2}$& $9.47^{+0.10}_{-0.10}$ & 88 & 0 & -- \\[0.20em]
SNF20070427-001 & $-0.03\pm{0.12}$ & $0.0777$ & $-0.12\pm{0.03}$ & $+0.69\pm{0.19}$ & $7.70^{+0.20}_{-0.20}$ &$-4.00^{+0.36}_{-0.59}$&$-11.7^{+0.4}_{-0.6}$& $10.54^{+0.10}_{-0.10}$ & 0 & 100 & -- \\[0.20em]
SNF20070429-000 & $-0.09\pm{0.12}$ & $0.0671$ & $-0.04\pm{0.03}$ & $-0.87\pm{0.10}$ & $7.91^{+0.12}_{-0.11}$ &$-2.52^{+0.02}_{-0.02}$&$-10.4^{+0.1}_{-0.1}$& $10.13^{+0.10}_{-0.10}$ & 99 & 90 & -- \\[0.20em]
SNF20070506-006 & $-0.11\pm{0.13}$ & $0.0355$ & $-0.04\pm{0.03}$ & $+1.19\pm{0.10}$ & $7.47^{+0.11}_{-0.12}$ &$-2.69^{+0.01}_{-0.01}$&$-10.2^{+0.1}_{-0.1}$& $9.88^{+0.10}_{-0.10}$ & 100 & 11 & -- \\[0.20em]
SNF20070531-011 & $-0.03\pm{0.13}$ & $0.0359$ & $-0.06\pm{0.03}$ & $-1.60\pm{0.20}$ & $8.55^{+0.10}_{-0.10}$ &$-2.63^{+0.02}_{-0.02}$&$-11.2^{+0.1}_{-0.1}$& $10.83^{+0.10}_{-0.10}$ & 0 & 100 & -- \\[0.20em]
SNF20070630-006 & $+0.03\pm{0.12}$ & $0.0706$ & $-0.04\pm{0.03}$ & $+0.38\pm{0.11}$ & $7.86^{+0.15}_{-0.15}$ &$-2.66^{+0.03}_{-0.03}$&$-10.5^{+0.1}_{-0.1}$& $9.66^{+0.10}_{-0.10}$ & 97 & 0 & -- \\[0.20em]
SNF20070701-005 & $-0.33\pm{0.12}$ & $0.0684$ & $+0.01\pm{0.03}$ & $+0.07\pm{0.16}$ & $8.42^{+0.12}_{-0.11}$ &$-2.71^{+0.03}_{-0.03}$&$-11.1^{+0.1}_{-0.1}$& $10.76^{+0.10}_{-0.10}$ & 0 & 100 & -- \\[0.20em]
SNF20070712-000 & $+0.02\pm{0.14}$ & $0.0298$ & $-0.02\pm{0.03}$ & $-0.03\pm{0.16}$ & $8.02^{+0.10}_{-0.10}$ &$-2.34^{+0.01}_{-0.01}$&$-10.4^{+0.1}_{-0.1}$& $9.95^{+0.10}_{-0.10}$ & 100 & 29 & -- \\[0.20em]
SNF20070712-003 & $+0.00\pm{0.12}$ & $0.0738$ & $-0.03\pm{0.03}$ & $+0.59\pm{0.18}$ & $7.67^{+0.18}_{-0.18}$ &$-3.71^{+0.23}_{-0.42}$&$-11.4^{+0.3}_{-0.5}$& $8.09^{+0.14}_{-0.14}$ & 1 & 0 & -- \\[0.20em]
SNF20070714-007 & $-0.16\pm{0.12}$ & $0.0417$ & $+0.25\pm{0.03}$ & $-1.17\pm{0.11}$ & $8.24^{+0.10}_{-0.10}$ &$-2.57^{+0.02}_{-0.02}$&$-10.8^{+0.1}_{-0.1}$& $10.43^{+0.10}_{-0.10}$ & 54 & 100 & -- \\[0.20em]
SNF20070725-001 & $+0.09\pm{0.12}$ & $0.0669$ & $-0.11\pm{0.03}$ & $+0.71\pm{0.15}$ & $7.19^{+0.30}_{-0.34}$ &$-2.81^{+0.04}_{-0.05}$&$-10.0^{+0.3}_{-0.3}$& $9.13^{+0.10}_{-0.10}$ & 99 & 0 & -- \\[0.20em]
SNF20070727-016 & $-0.28\pm{0.13}$ & $0.0661$ & $-0.08\pm{0.03}$ & $+0.28\pm{0.11}$ & $7.58^{+0.23}_{-0.24}$ &$-4.28^{+0.47}_{-0.60}$&$-11.9^{+0.5}_{-0.7}$& $10.75^{+0.10}_{-0.10}$ & 1 & 100 & -- \\[0.20em]
SNF20070802-000 & $-0.05\pm{0.12}$ & $0.0648$ & $+0.06\pm{0.03}$ & $+0.06\pm{0.15}$ & $7.78^{+0.19}_{-0.20}$ &$-4.24^{+0.49}_{-0.62}$&$-12.0^{+0.5}_{-0.7}$& $11.30^{+0.10}_{-0.10}$ & 0 & 100 & -- \\[0.20em]
SNF20070806-026 & $+0.08\pm{0.13}$ & $0.0440$ & $-0.09\pm{0.03}$ & $-1.72\pm{0.14}$ & $7.74^{+0.17}_{-0.17}$ &$-4.32^{+0.35}_{-0.54}$&$-12.1^{+0.4}_{-0.6}$& $10.81^{+0.10}_{-0.10}$ & 0 & 100 & -- \\[0.20em]
SNF20070818-001 & $-0.13\pm{0.12}$ & $0.0734$ & $+0.05\pm{0.03}$ & $+0.18\pm{0.16}$ & $7.66^{+0.25}_{-0.26}$ &$-3.24^{+0.12}_{-0.17}$&$-10.9^{+0.3}_{-0.3}$& $10.27^{+0.10}_{-0.10}$ & 36 & 99 & -- \\[0.20em]
SNF20070820-000 & $+0.00\pm{0.12}$ & $0.0687$ & $+0.08\pm{0.03}$ & $-0.31\pm{0.13}$ & $8.59^{+0.10}_{-0.11}$ &$-2.01^{+0.01}_{-0.01}$&$-10.6^{+0.1}_{-0.1}$& $10.16^{+0.10}_{-0.10}$ & 98 & 94 & -- \\[0.20em]
SNF20070831-015 & $+0.11\pm{0.12}$ & $0.0674$ & $-0.02\pm{0.03}$ & $+1.93\pm{0.18}$ & $8.60^{+0.10}_{-0.11}$ &$-2.04^{+0.01}_{-0.01}$&$-10.6^{+0.1}_{-0.1}$& $10.07^{+0.10}_{-0.10}$ & 95 & 75 & -- \\[0.20em]
SNF20070902-018 & $+0.07\pm{0.12}$ & $0.0680$ & $+0.04\pm{0.03}$ & $-0.69\pm{0.09}$ & $8.62^{+0.11}_{-0.11}$ &$-2.27^{+0.01}_{-0.01}$&$-10.9^{+0.1}_{-0.1}$& $10.34^{+0.10}_{-0.10}$ & 26 & 99 & -- \\[0.20em]
SNF20070902-021 & $-0.11\pm{0.12}$ & $0.0740$ & $+0.01\pm{0.03}$ & $-0.16\pm{0.10}$ & $8.14^{+0.17}_{-0.18}$ &$-2.24^{+0.01}_{-0.01}$&$-10.4^{+0.2}_{-0.2}$& $9.53^{+0.10}_{-0.10}$ & 99 & 0 & -- \\[0.20em]
SNF20071003-004 & $+0.13\pm{0.13}$ & $0.0762$ & $-0.03\pm{0.03}$ & $+1.19\pm{0.34}$ & $7.48^{+0.24}_{-0.25}$ &$-3.27^{+0.09}_{-0.12}$&$-10.8^{+0.3}_{-0.3}$& $9.17^{+0.10}_{-0.11}$ & 59 & 0 & -- \\[0.20em]
SNF20071003-016 & $+0.11\pm{0.12}$ & $0.0547$ & $+0.09\pm{0.03}$ & $-0.09\pm{0.14}$ & $8.52^{+0.11}_{-0.11}$ &$-2.39^{+0.02}_{-0.02}$&$-10.9^{+0.1}_{-0.1}$& $8.95^{+0.10}_{-0.10}$ & 22 & 0 & -- \\[0.20em]
SNF20071015-000 & $+0.25\pm{0.13}$ & $0.0374$ & $+0.33\pm{0.03}$ & $+1.03\pm{0.27}$ & $8.36^{+0.10}_{-0.10}$ &$-2.28^{+0.01}_{-0.01}$&$-10.6^{+0.1}_{-0.1}$& $10.68^{+0.10}_{-0.10}$ & 96 & 100 & -- \\[0.20em]
SNF20071021-000 & $-0.02\pm{0.14}$ & $0.0264$ & $+0.04\pm{0.03}$ & $-0.56\pm{0.17}$ & $7.80^{+0.11}_{-0.11}$ &$-2.51^{+0.01}_{-0.01}$&$-10.3^{+0.1}_{-0.1}$& $9.68^{+0.10}_{-0.10}$ & 100 & 0 & -- \\[0.20em]
SNF20071108-021 & $-0.18\pm{0.12}$ & $0.0741$ & $-0.02\pm{0.03}$ & $+0.95\pm{0.17}$ & $7.77^{+0.17}_{-0.17}$ &$-3.30^{+0.07}_{-0.08}$&$-11.1^{+0.2}_{-0.2}$& $9.12^{+0.11}_{-0.10}$ & 8 & 0 & -- \\[0.20em]
SNF20080507-000 & $-0.17\pm{0.12}$ & $0.0540$ & $+0.06\pm{0.03}$ & $+0.90\pm{0.22}$ & $8.90^{+0.10}_{-0.10}$ &$-1.94^{+0.01}_{-0.01}$&$-10.8^{+0.1}_{-0.1}$& $10.12^{+0.10}_{-0.10}$ & 42 & 88 & -- \\[0.20em]
SNF20080510-001 & $+0.07\pm{0.12}$ & $0.0725$ & $-0.06\pm{0.03}$ & $+0.46\pm{0.18}$ & $7.25^{+0.31}_{-0.36}$ &$-3.59^{+0.21}_{-0.31}$&$-10.9^{+0.5}_{-0.4}$& $8.54^{+0.65}_{-0.55}$ & 45 & 0 & -- \\[0.20em]
SNF20080512-008 & $-0.07\pm{0.12}$ & $0.0774$ & $-0.04\pm{0.03}$ & $+0.91\pm{0.15}$ & $7.17^{+0.32}_{-0.41}$ &$-3.45^{+0.14}_{-0.25}$&$-10.7^{+0.5}_{-0.4}$& $7.97^{+0.20}_{-0.22}$ & 65 & 0 & -- \\[0.20em]
SNF20080512-010 & $-0.09\pm{0.14}$ & $0.0632$ & $-0.02\pm{0.03}$ & $-1.40\pm{0.26}$ & $8.91^{+0.11}_{-0.10}$ &$-4.07^{+0.34}_{-0.53}$&$-13.0^{+0.3}_{-0.5}$& $11.71^{+0.10}_{-0.10}$ & 0 & 100 & -- \\[0.20em]
SNF20080514-002 & $+0.17\pm{0.15}$ & $0.0229$ & $-0.12\pm{0.03}$ & $-1.64\pm{0.10}$ & $8.64^{+0.10}_{-0.10}$ &$-3.54^{+0.07}_{-0.07}$&$-12.2^{+0.1}_{-0.1}$& $10.69^{+0.10}_{-0.10}$ & 0 & 100 & -- \\[0.20em]
SNF20080516-000 & $+0.04\pm{0.12}$ & $0.0733$ & $-0.04\pm{0.03}$ & $+1.33\pm{0.21}$ & $7.69^{+0.16}_{-0.16}$ &$-2.85^{+0.04}_{-0.04}$&$-10.5^{+0.2}_{-0.2}$& $8.78^{+0.12}_{-0.12}$ & 95 & 0 & -- \\[0.20em]
SNF20080516-022 & $+0.04\pm{0.12}$ & $0.0746$ & $-0.07\pm{0.03}$ & $+0.15\pm{0.13}$ & $7.32^{+0.30}_{-0.37}$ &$-3.67^{+0.16}_{-0.27}$&$-11.0^{+0.4}_{-0.4}$& $10.62^{+0.10}_{-0.10}$ & 31 & 100 & -- \\[0.20em]
SNF20080522-011 & $-0.06\pm{0.13}$ & $0.0383$ & $-0.08\pm{0.03}$ & $+0.83\pm{0.17}$ & $8.09^{+0.10}_{-0.10}$ &$-2.15^{+0.01}_{-0.01}$&$-10.2^{+0.1}_{-0.1}$& $8.62^{+0.10}_{-0.10}$ & 100 & 0 & -- \\[0.20em]
SNF20080531-000 & $+0.05\pm{0.13}$ & $0.0368$ & $-0.04\pm{0.03}$ & $-0.51\pm{0.17}$ & $7.85^{+0.10}_{-0.11}$ &$-2.12^{+0.01}_{-0.01}$&$-10.0^{+0.1}_{-0.1}$& $10.00^{+0.10}_{-0.10}$ & 100 & 48 & -- \\[0.20em]
SNF20080610-000 & $+0.09\pm{0.13}$ & $0.0788$ & $-0.01\pm{0.03}$ & $+0.13\pm{0.16}$ & $7.68^{+0.20}_{-0.19}$ &$-3.28^{+0.11}_{-0.14}$&$-11.0^{+0.2}_{-0.2}$& $8.91^{+0.11}_{-0.11}$ & 25 & 0 & -- \\[0.20em]
SNF20080612-003 & $-0.24\pm{0.13}$ & $0.0328$ & $-0.03\pm{0.03}$ & $+0.73\pm{0.17}$ & $8.52^{+0.10}_{-0.11}$ &$-2.64^{+0.01}_{-0.01}$&$-11.2^{+0.1}_{-0.1}$& $9.91^{+0.10}_{-0.10}$ & 0 & 19 & -- \\[0.20em]
SNF20080614-010 & $-0.15\pm{0.13}$ & $0.0751$ & $+0.00\pm{0.03}$ & $-2.33\pm{0.14}$ & $8.14^{+0.15}_{-0.15}$ &$-4.02^{+0.32}_{-0.52}$&$-12.2^{+0.4}_{-0.5}$& $10.56^{+0.10}_{-0.10}$ & 0 & 100 & -- \\[0.20em]
SNF20080620-000 & $+0.07\pm{0.13}$ & $0.0332$ & $+0.01\pm{0.03}$ & $-0.90\pm{0.14}$ & $8.54^{+0.10}_{-0.10}$ &$-1.99^{+0.01}_{-0.01}$&$-10.5^{+0.1}_{-0.1}$& $8.98^{+0.10}_{-0.10}$ & 99 & 0 & -- \\[0.20em]
SNF20080623-001 & $+0.20\pm{0.12}$ & $0.0448$ & $-0.07\pm{0.03}$ & $+0.00\pm{0.12}$ & $7.09^{+0.32}_{-0.39}$ &$-3.30^{+0.08}_{-0.09}$&$-10.4^{+0.4}_{-0.4}$& $8.81^{+0.10}_{-0.10}$ & 90 & 0 & -- \\[0.20em]
SNF20080717-000 & $-0.03\pm{0.12}$ & $0.0586$ & $+0.18\pm{0.03}$ & $+0.62\pm{0.12}$ & $8.88^{+0.10}_{-0.10}$ &$-1.96^{+0.01}_{-0.01}$&$-10.8^{+0.1}_{-0.1}$& $10.38^{+0.10}_{-0.10}$ & 41 & 100 & -- \\[0.20em]
SNF20080725-004 & $+0.07\pm{0.12}$ & $0.0539$ & $-0.00\pm{0.03}$ & $+0.59\pm{0.12}$ & $8.56^{+0.10}_{-0.10}$ &$-1.93^{+0.01}_{-0.01}$&$-10.5^{+0.1}_{-0.1}$& $9.83^{+0.10}_{-0.10}$ & 99 & 4 & -- \\[0.20em]
SNF20080731-000 & $-0.16\pm{0.13}$ & $0.0755$ & $+0.07\pm{0.03}$ & $-1.31\pm{0.11}$ & $8.22^{+0.17}_{-0.18}$ &$-3.64^{+0.25}_{-0.45}$&$-11.9^{+0.3}_{-0.5}$& $9.99^{+0.10}_{-0.10}$ & 0 & 47 & -- \\[0.20em]
SNF20080802-006 & $-0.07\pm{0.13}$ & $0.0711$ & $-0.00\pm{0.03}$ & $-1.66\pm{0.11}$ & $8.02^{+0.17}_{-0.17}$ &$-3.84^{+0.28}_{-0.48}$&$-11.9^{+0.3}_{-0.5}$& $10.69^{+0.10}_{-0.10}$ & 0 & 100 & -- \\[0.20em]
SNF20080803-000 & $-0.03\pm{0.12}$ & $0.0568$ & $+0.11\pm{0.03}$ & $+0.37\pm{0.13}$ & $8.31^{+0.11}_{-0.11}$ &$-2.94^{+0.04}_{-0.05}$&$-11.2^{+0.1}_{-0.1}$& $10.66^{+0.10}_{-0.10}$ & 0 & 100 & -- \\[0.20em]
SNF20080806-002 & $-0.07\pm{0.12}$ & $0.0610$ & $+0.04\pm{0.03}$ & $+0.75\pm{0.15}$ & $8.72^{+0.10}_{-0.11}$ &$-1.92^{+0.01}_{-0.01}$&$-10.6^{+0.1}_{-0.1}$& $10.36^{+0.10}_{-0.10}$ & 95 & 100 & -- \\[0.20em]
SNF20080810-001 & $+0.02\pm{0.12}$ & $0.0424$ & $-0.02\pm{0.03}$ & $-0.90\pm{0.10}$ & $7.50^{+0.20}_{-0.21}$ &$-4.05^{+0.29}_{-0.50}$&$-11.6^{+0.4}_{-0.5}$& $10.51^{+0.11}_{-0.10}$ & 1 & 100 & -- \\[0.20em]
SNF20080815-017 & $+0.02\pm{0.14}$ & $0.0637$ & $-0.02\pm{0.03}$ & $-1.82\pm{0.16}$ & $8.41^{+0.12}_{-0.13}$ &$-4.11^{+0.37}_{-0.61}$&$-12.5^{+0.4}_{-0.6}$& $11.12^{+0.10}_{-0.10}$ & 0 & 100 & -- \\[0.20em]
SNF20080821-000 & $-0.12\pm{0.12}$ & $0.0737$ & $+0.02\pm{0.03}$ & $+0.52\pm{0.17}$ & $8.76^{+0.10}_{-0.10}$ &$-2.12^{+0.01}_{-0.01}$&$-10.9^{+0.1}_{-0.1}$& $10.53^{+0.10}_{-0.10}$ & 28 & 100 & -- \\[0.20em]
SNF20080822-005 & $-0.19\pm{0.12}$ & $0.0696$ & $-0.03\pm{0.03}$ & $+0.71\pm{0.23}$ & $8.22^{+0.13}_{-0.13}$ &$-2.69^{+0.03}_{-0.03}$&$-10.9^{+0.1}_{-0.1}$& $10.92^{+0.10}_{-0.09}$ & 24 & 100 & -- \\[0.20em]
SNF20080825-010 & $-0.22\pm{0.13}$ & $0.0401$ & $-0.03\pm{0.03}$ & $-0.81\pm{0.17}$ & $8.51^{+0.11}_{-0.11}$ &$-3.95^{+0.24}_{-0.41}$&$-12.5^{+0.3}_{-0.4}$& $10.92^{+0.10}_{-0.10}$ & 0 & 100 & -- \\[0.20em]
SNF20080908-000 & $+0.02\pm{0.12}$ & $0.0514$ & $-0.10\pm{0.03}$ & $+0.18\pm{0.20}$ & $7.46^{+0.17}_{-0.17}$ &$-2.69^{+0.02}_{-0.02}$&$-10.2^{+0.2}_{-0.2}$& $8.41^{+0.11}_{-0.11}$ & 100 & 0 & -- \\[0.20em]
SNF20080909-030 & $-0.04\pm{0.13}$ & $0.0301$ & $+0.01\pm{0.03}$ & $+1.20\pm{0.13}$ & $6.90^{+0.16}_{-0.17}$ &$-2.71^{+0.02}_{-0.02}$&$-9.6^{+0.2}_{-0.2}$& $9.23^{+0.10}_{-0.10}$ & 100 & 0 & -- \\[0.20em]
SNF20080913-031 & $-0.08\pm{0.14}$ & $0.0543$ & $+0.01\pm{0.03}$ & $+0.06\pm{0.19}$ & $7.36^{+0.26}_{-0.27}$ &$-4.02^{+0.29}_{-0.49}$&$-11.4^{+0.4}_{-0.5}$& $10.52^{+0.10}_{-0.10}$ & 8 & 100 & -- \\[0.20em]
SNF20080914-001 & $-0.08\pm{0.15}$ & $0.0235$ & $+0.13\pm{0.03}$ & $-0.07\pm{0.14}$ & $8.47^{+0.10}_{-0.10}$ &$-2.69^{+0.01}_{-0.01}$&$-11.2^{+0.1}_{-0.1}$& $10.00^{+0.10}_{-0.10}$ & 0 & 51 & -- \\[0.20em]
SNF20080918-000 & $+0.10\pm{0.12}$ & $0.0653$ & $+0.12\pm{0.03}$ & $+1.38\pm{0.24}$ & $7.80^{+0.14}_{-0.15}$ &$-2.76^{+0.02}_{-0.02}$&$-10.6^{+0.1}_{-0.1}$& $10.22^{+0.10}_{-0.10}$ & 95 & 98 & -- \\[0.20em]
SNF20080919-001 & $-0.33\pm{0.13}$ & $0.0411$ & $-0.00\pm{0.03}$ & $+0.84\pm{0.16}$ & $8.09^{+0.16}_{-0.15}$ &$-2.86^{+0.03}_{-0.03}$&$-10.9^{+0.1}_{-0.2}$& $8.30^{+0.12}_{-0.12}$ & 20 & 0 & -- \\[0.20em]
SNF20080919-002 & $+0.13\pm{0.12}$ & $0.0548$ & $+0.05\pm{0.03}$ & $-1.59\pm{0.13}$ & $7.89^{+0.13}_{-0.13}$ &$-2.73^{+0.02}_{-0.02}$&$-10.6^{+0.1}_{-0.1}$& $9.95^{+0.10}_{-0.10}$ & 93 & 32 & -- \\[0.20em]
SNF20080920-000 & $-0.06\pm{0.13}$ & $0.0395$ & $-0.01\pm{0.03}$ & $+1.01\pm{0.23}$ & $8.31^{+0.10}_{-0.10}$ &$-2.21^{+0.01}_{-0.01}$&$-10.5^{+0.1}_{-0.1}$& $9.65^{+0.10}_{-0.10}$ & 99 & 0 & -- \\[0.20em]
SNF20080926-009 & $-0.19\pm{0.12}$ & $0.0713$ & $-0.01\pm{0.03}$ & $+0.22\pm{0.10}$ & $7.46^{+0.32}_{-0.38}$ &$-4.19^{+0.36}_{-0.62}$&$-11.7^{+0.5}_{-0.7}$& $9.14^{+0.10}_{-0.11}$ & 6 & 0 & -- \\[0.20em]
CSS120424\_01 & $+0.09\pm{0.13}$ & $0.0372$ & $-0.07\pm{0.03}$ & $+0.85\pm{0.17}$ & $6.96^{+0.22}_{-0.24}$ &$-3.61^{+0.10}_{-0.12}$&$-10.6^{+0.3}_{-0.2}$& $10.18^{+0.10}_{-0.10}$ & 82 & 95 & 1 \\[0.20em]
CSS130502\_01 & $+0.18\pm{0.13}$ & $0.0338$ & $-0.10\pm{0.03}$ & $+0.02\pm{0.23}$ & $7.15^{+0.22}_{-0.22}$ &$-3.30^{+0.07}_{-0.08}$&$-10.4^{+0.2}_{-0.2}$& $9.17^{+0.10}_{-0.10}$ & 94 & 0 & 1 \\[0.20em]
LSQ12ekl & $+0.03\pm{0.12}$ & $0.0752$* & $-0.01\pm{0.03}$ & $-0.37\pm{0.13}$ & $7.57^{+0.22}_{-0.22}$ &$-2.17^{+0.01}_{-0.01}$&$-9.8^{+0.2}_{-0.2}$& $9.57^{+0.10}_{-0.10}$ & 100 & 0 & -- \\[0.20em]
LSQ12fmx & $+0.05\pm{0.13}$ & $0.0668$ & $-0.04\pm{0.03}$ & $-1.30\pm{0.19}$ & $7.14^{+0.33}_{-0.42}$ &$-3.29^{+0.16}_{-0.24}$&$-10.4^{+0.5}_{-0.4}$& $10.27^{+0.10}_{-0.10}$ & 81 & 99 & -- \\[0.20em]
LSQ13vy & $+0.01\pm{0.13}$ & $0.0426$* & $+0.04\pm{0.03}$ & $-1.25\pm{0.11}$ & $7.83^{+0.12}_{-0.12}$ &$-2.88^{+0.03}_{-0.03}$&$-10.7^{+0.1}_{-0.1}$& $10.43^{+0.10}_{-0.10}$ & 79 & 100 & -- \\[0.20em]
PTF09dlc & $+0.02\pm{0.12}$ & $0.0661$ & $-0.06\pm{0.03}$ & $+0.11\pm{0.11}$ & $7.27^{+0.18}_{-0.20}$ &$-3.04^{+0.05}_{-0.05}$&$-10.3^{+0.2}_{-0.2}$& $8.74^{+0.11}_{-0.11}$ & 99 & 0 & 2 \\[0.20em]
PTF09dnl & $-0.14\pm{0.15}$ & $0.0232$ & $+0.04\pm{0.03}$ & $+0.69\pm{0.10}$ & $7.62^{+0.11}_{-0.11}$ &$-2.87^{+0.01}_{-0.01}$&$-10.5^{+0.1}_{-0.1}$& $7.93^{+0.11}_{-0.11}$ & 99 & 0 & 2 \\[0.20em]
PTF09dnp & $-0.19\pm{0.13}$ & $0.0374$ & $-0.04\pm{0.03}$ & $-0.84\pm{0.24}$ & $7.57^{+0.15}_{-0.15}$ &$-4.62^{+0.38}_{-0.57}$&$-12.2^{+0.4}_{-0.6}$& $10.71^{+0.10}_{-0.10}$ & 0 & 100 & 2 \\[0.20em]
PTF09foz & $-0.17\pm{0.12}$ & $0.0533$ & $-0.02\pm{0.03}$ & $-1.24\pm{0.25}$ & $8.70^{+0.10}_{-0.10}$ &$-4.60^{+0.41}_{-0.53}$&$-13.3^{+0.4}_{-0.5}$& $10.54^{+0.10}_{-0.10}$ & 0 & 100 & 2 \\[0.20em]
PTF10hmv & $+0.35\pm{0.13}$ & $0.0322$ & $+0.12\pm{0.03}$ & $+1.35\pm{0.14}$ & $7.96^{+0.11}_{-0.11}$ &$-2.65^{+0.02}_{-0.02}$&$-10.6^{+0.1}_{-0.1}$& $8.28^{+0.10}_{-0.10}$ & 97 & 0 & 3 \\[0.20em]
PTF10mwb & $+0.13\pm{0.15}$ & $0.0312$ & $-0.03\pm{0.03}$ & $-0.69\pm{0.10}$ & $7.98^{+0.11}_{-0.10}$ &$-3.10^{+0.03}_{-0.03}$&$-11.1^{+0.1}_{-0.1}$& $9.01^{+0.10}_{-0.10}$ & 1 & 0 & 2 \\[0.20em]
PTF10qjl & $+0.11\pm{0.12}$ & $0.0576$ & $-0.06\pm{0.03}$ & $+1.27\pm{0.14}$ & $7.51^{+0.14}_{-0.14}$ &$-2.06^{+0.01}_{-0.01}$&$-9.6^{+0.1}_{-0.1}$& $8.81^{+0.10}_{-0.10}$ & 100 & 0 & 2 \\[0.20em]
PTF10qjq & $-0.09\pm{0.14}$ & $0.0280$ & $+0.03\pm{0.03}$ & $-0.30\pm{0.10}$ & $8.97^{+0.10}_{-0.10}$ &$-1.21^{+0.01}_{-0.01}$&$-10.2^{+0.1}_{-0.1}$& $9.75^{+0.10}_{-0.10}$ & 100 & 0 & 2 \\[0.20em]
PTF10tce & $-0.00\pm{0.12}$ & $0.0397$ & $+0.01\pm{0.03}$ & $+0.47\pm{0.12}$ & $7.68^{+0.15}_{-0.15}$ &$-3.81^{+0.33}_{-0.55}$&$-11.5^{+0.3}_{-0.6}$& $10.16^{+0.10}_{-0.10}$ & 1 & 94 & 3 \\[0.20em]
PTF10wnm & $+0.02\pm{0.12}$ & $0.0648$* & $-0.02\pm{0.03}$ & $+0.66\pm{0.15}$ & $8.17^{+0.11}_{-0.11}$ &$-2.53^{+0.03}_{-0.03}$&$-10.7^{+0.1}_{-0.1}$& $10.22^{+0.10}_{-0.10}$ & 83 & 98 & 2 \\[0.20em]
PTF10wof & $+0.12\pm{0.12}$ & $0.0513$ & $+0.00\pm{0.03}$ & $+0.17\pm{0.12}$ & $7.82^{+0.12}_{-0.13}$ &$-2.87^{+0.05}_{-0.05}$&$-10.7^{+0.1}_{-0.1}$& $9.69^{+0.10}_{-0.10}$ & 83 & 0 & 2 \\[0.20em]
PTF10xyt & $+0.37\pm{0.13}$ & $0.0476$* & $+0.11\pm{0.03}$ & $-0.11\pm{0.20}$ & $8.74^{+0.10}_{-0.10}$ &$-1.84^{+0.01}_{-0.01}$&$-10.6^{+0.1}_{-0.1}$& $9.26^{+0.10}_{-0.10}$ & 99 & 0 & 3 \\[0.20em]
PTF10zdk & $+0.09\pm{0.13}$ & $0.0317$* & $+0.07\pm{0.03}$ & $+0.22\pm{0.16}$ & $8.38^{+0.10}_{-0.10}$ &$-2.09^{+0.01}_{-0.01}$&$-10.5^{+0.1}_{-0.1}$& $9.29^{+0.10}_{-0.10}$ & 99 & 0 & 2 \\[0.20em]
PTF11bnx & $+0.18\pm{0.12}$ & $0.0553$ & $+0.07\pm{0.03}$ & $-0.06\pm{0.17}$ & $7.56^{+0.12}_{-0.12}$ &$-1.86^{+0.01}_{-0.01}$&$-9.4^{+0.1}_{-0.1}$& $9.50^{+0.10}_{-0.10}$ & 100 & 0 & 6 \\[0.20em]
PTF11cao & $+0.04\pm{0.13}$ & $0.0402$ & $+0.05\pm{0.03}$ & $+0.23\pm{0.13}$ & $7.85^{+0.11}_{-0.11}$ &$-2.69^{+0.03}_{-0.03}$&$-10.6^{+0.1}_{-0.1}$& $9.62^{+0.10}_{-0.10}$ & 99 & 0 & 6 \\[0.20em]
PTF11mty & $+0.02\pm{0.12}$ & $0.0755$* & $-0.06\pm{0.03}$ & $+0.83\pm{0.15}$ & $9.12^{+0.10}_{-0.10}$ &$-0.89^{+0.01}_{-0.01}$&$-10.0^{+0.1}_{-0.1}$& $9.81^{+0.10}_{-0.10}$ & 100 & 3 & 6 \\[0.20em]
PTF11pbp & $-0.11\pm{0.14}$ & $0.0277$ & $+0.02\pm{0.03}$ & $+0.09\pm{0.13}$ & $8.05^{+0.11}_{-0.11}$ &$-3.10^{+0.03}_{-0.03}$&$-11.2^{+0.1}_{-0.1}$& $10.83^{+0.09}_{-0.10}$ & 0 & 100 & 5 \\[0.20em]
PTF12dxm & $-0.03\pm{0.12}$ & $0.0638$ & $+0.04\pm{0.03}$ & $-2.21\pm{0.18}$ & $7.85^{+0.18}_{-0.22}$ &$-3.95^{+0.26}_{-0.44}$&$-11.8^{+0.3}_{-0.5}$& $11.19^{+0.10}_{-0.10}$ & 0 & 100 & 6 \\[0.20em]
PTF12iiq & $-0.00\pm{0.14}$ & $0.0284$ & $-0.00\pm{0.03}$ & $-1.42\pm{0.10}$ & $8.74^{+0.10}_{-0.10}$ &$-4.13^{+0.24}_{-0.41}$&$-12.9^{+0.3}_{-0.4}$& $10.66^{+0.10}_{-0.10}$ & 0 & 100 & 4 \\[0.20em]
SN2004ef & $-0.10\pm{0.18}$ & $0.0296$ & $+0.05\pm{0.03}$ & $-1.60\pm{0.17}$ & $8.48^{+0.10}_{-0.10}$ &$-2.90^{+0.02}_{-0.02}$&$-11.4^{+0.1}_{-0.1}$& $10.98^{+0.10}_{-0.10}$ & 0 & 100 & 7 \\[0.20em]
SN2004gc & $-0.22\pm{0.13}$ & $0.0320$ & $+0.05\pm{0.03}$ & $-0.46\pm{0.11}$ & $9.14^{+0.10}_{-0.10}$ &$-1.74^{+0.01}_{-0.01}$&$-10.9^{+0.1}_{-0.1}$& $10.20^{+0.10}_{-0.10}$ & 29 & 97 & 8 \\[0.20em]
SN2005hc & $+0.12\pm{0.13}$ & $0.0453$ & $-0.05\pm{0.03}$ & $+0.89\pm{0.28}$ & $8.28^{+0.11}_{-0.11}$ &$-2.87^{+0.05}_{-0.05}$&$-11.1^{+0.1}_{-0.1}$& $10.72^{+0.10}_{-0.10}$ & 0 & 100 & 9 \\[0.20em]
SN2005hj & $-0.14\pm{0.13}$ & $0.0563$ & $+0.06\pm{0.03}$ & $+1.96\pm{0.49}$ & $8.47^{+0.10}_{-0.11}$ &$-2.06^{+0.01}_{-0.01}$&$-10.5^{+0.1}_{-0.1}$& $9.60^{+0.10}_{-0.10}$ & 99 & 0 & 10 \\[0.20em]
SN2005ir & $-0.09\pm{0.14}$ & $0.0752$ & $+0.04\pm{0.04}$ & $+1.66\pm{0.68}$ & $8.41^{+0.10}_{-0.11}$ &$-1.75^{+0.01}_{-0.01}$&$-10.2^{+0.1}_{-0.1}$& $10.28^{+0.10}_{-0.10}$ & 100 & 99 & 9 \\[0.20em]
SN2006cj & $-0.03\pm{0.12}$ & $0.0683$ & $-0.03\pm{0.03}$ & $+0.48\pm{0.18}$ & $8.05^{+0.12}_{-0.12}$ &$-2.90^{+0.04}_{-0.05}$&$-11.0^{+0.1}_{-0.1}$& $10.66^{+0.10}_{-0.10}$ & 14 & 100 & 11 \\[0.20em]
SN2006dm & $+0.11\pm{0.16}$ & $0.0208$ & $-0.02\pm{0.03}$ & $-1.86\pm{0.29}$ & $8.18^{+0.11}_{-0.11}$ &$-4.08^{+0.23}_{-0.37}$&$-12.3^{+0.3}_{-0.4}$& $11.15^{+0.10}_{-0.10}$ & 0 & 100 & 12 \\[0.20em]
SN2006do & $-0.12\pm{0.15}$ & $0.0274$ & $-0.04\pm{0.03}$ & $-2.53\pm{0.45}$ & $9.10^{+0.10}_{-0.10}$ &$-4.39^{+0.38}_{-0.63}$&$-13.5^{+0.4}_{-0.7}$& $10.79^{+0.10}_{-0.10}$ & 0 & 100 & 12 \\[0.20em]
SN2006ob & $-0.15\pm{0.13}$ & $0.0582$ & $-0.02\pm{0.03}$ & $-2.57\pm{0.24}$ & $8.83^{+0.11}_{-0.11}$ &$-3.93^{+0.27}_{-0.45}$&$-12.8^{+0.3}_{-0.5}$& $11.38^{+0.10}_{-0.10}$ & 0 & 100 & 9 \\[0.20em]
SN2007bc & $-0.11\pm{0.15}$ & $0.0219$ & $-0.02\pm{0.03}$ & $-0.81\pm{0.24}$ & $7.74^{+0.12}_{-0.12}$ &$-5.62^{+1.04}_{-1.24}$&$-13.4^{+1.0}_{-1.2}$& $10.96^{+0.10}_{-0.10}$ & 0 & 100 & 12 \\[0.20em]
SN2007bd & $+0.04\pm{0.14}$ & $0.0314$ & $-0.07\pm{0.03}$ & $-0.52\pm{0.35}$ & $8.65^{+0.10}_{-0.10}$ &$-2.25^{+0.01}_{-0.01}$&$-10.9^{+0.1}_{-0.1}$& $10.98^{+0.10}_{-0.10}$ & 20 & 100 & 12 \\[0.20em]
SN2007cq & $-0.17\pm{0.14}$ & $0.0248$ & $-0.08\pm{0.03}$ & $-0.40\pm{0.15}$ & $8.02^{+0.10}_{-0.10}$ &$-2.79^{+0.03}_{-0.03}$&$-10.8^{+0.1}_{-0.1}$& $9.74^{+0.10}_{-0.10}$ & 52 & 0 & 13 \\[0.20em]
SN2007kk & $-0.15\pm{0.12}$ & $0.0407$ & $-0.04\pm{0.03}$ & $+0.54\pm{0.15}$ & $8.35^{+0.11}_{-0.11}$ &$-3.09^{+0.05}_{-0.05}$&$-11.4^{+0.1}_{-0.1}$& $11.32^{+0.10}_{-0.10}$ & 0 & 100 & 12 \\[0.20em]
SN2007nq & $-0.18\pm{0.13}$ & $0.0439$ & $-0.02\pm{0.03}$ & $-1.98\pm{0.22}$ & $7.99^{+0.14}_{-0.14}$ &$-3.27^{+0.07}_{-0.09}$&$-11.3^{+0.2}_{-0.2}$& $11.51^{+0.10}_{-0.10}$ & 0 & 100 & 10 \\[0.20em]
SN2009hi & $-0.05\pm{0.13}$ & $0.0399$ & $+0.15\pm{0.03}$ & $-2.30\pm{0.09}$ & $8.39^{+0.11}_{-0.11}$ &$-4.13^{+0.49}_{-0.79}$&$-12.5^{+0.5}_{-0.8}$& $11.73^{+0.10}_{-0.10}$ & 0 & 100 & 12 \\[0.20em]
SN2010dt & $+0.04\pm{0.12}$ & $0.0529$ & $-0.07\pm{0.03}$ & $-0.03\pm{0.09}$ & $7.37^{+0.20}_{-0.20}$ &$-3.37^{+0.07}_{-0.08}$&$-10.7^{+0.2}_{-0.2}$& $10.59^{+0.10}_{-0.10}$ & 64 & 100 & 12 \\[0.20em]
SN2010ex & $+0.27\pm{0.15}$ & $0.0216$ & $-0.07\pm{0.03}$ & $+0.38\pm{0.12}$ & $7.84^{+0.10}_{-0.11}$ &$-2.52^{+0.01}_{-0.01}$&$-10.4^{+0.1}_{-0.1}$& $9.72^{+0.10}_{-0.10}$ & 100 & 0 & 14 \\[0.20em]
SN2011bc & $-0.03\pm{0.15}$ & $0.0218$ & $+0.10\pm{0.03}$ & $+0.05\pm{0.10}$ & $8.77^{+0.10}_{-0.10}$ &$-2.35^{+0.01}_{-0.01}$&$-11.1^{+0.1}_{-0.1}$& $10.86^{+0.10}_{-0.10}$ & 0 & 100 & 15 \\[0.20em]
SN2011be & $+0.13\pm{0.13}$ & $0.0356$ & $-0.09\pm{0.03}$ & $+0.16\pm{0.23}$ & $7.85^{+0.11}_{-0.10}$ &$-2.55^{+0.01}_{-0.01}$&$-10.4^{+0.1}_{-0.1}$& $11.18^{+0.10}_{-0.10}$ & 100 & 100 & 1 \\[0.20em]
SN2011ga & $-0.03\pm{0.13}$ & $0.0381$ & $-0.06\pm{0.03}$ & $-0.28\pm{0.17}$ & $7.23^{+0.21}_{-0.22}$ &$-4.34^{+0.46}_{-0.93}$&$-11.6^{+0.6}_{-0.9}$& $10.61^{+0.10}_{-0.10}$ & 5 & 100 & 1 \\[0.20em]
SN2011ho & $+0.27\pm{0.14}$ & $0.0328$ & $+0.05\pm{0.03}$ & $-1.92\pm{0.17}$ & $8.67^{+0.10}_{-0.10}$ &$-4.69^{+0.44}_{-0.65}$&$-13.4^{+0.5}_{-0.7}$& $11.40^{+0.10}_{-0.10}$ & 0 & 100 & 1 \\[0.20em]
SN2011hv & $-0.02\pm{0.15}$ & $0.0285$ & $+0.47\pm{0.04}$ & $+1.12\pm{0.51}$ & $8.51^{+0.11}_{-0.10}$ &$-2.53^{+0.01}_{-0.01}$&$-11.0^{+0.1}_{-0.1}$& $10.71^{+0.10}_{-0.10}$ & 1 & 100 & 16 \\[0.20em]
SN2013be & $-0.23\pm{0.12}$ & $0.0670$ & $+0.04\pm{0.03}$ & $+0.43\pm{0.17}$ & $8.08^{+0.14}_{-0.14}$ &$-4.17^{+0.41}_{-0.71}$&$-12.3^{+0.5}_{-0.8}$& $10.90^{+0.10}_{-0.10}$ & 0 & 100 & 17 \\[0.20em]
SN2013bs & $+0.03\pm{0.14}$ & $0.0275$ & $-0.02\pm{0.03}$ & $-2.18\pm{0.21}$ & $6.70^{+0.31}_{-0.37}$ &$-5.22^{+0.40}_{-0.57}$&$-11.9^{+0.6}_{-0.7}$& $11.09^{+0.10}_{-0.10}$ & 2 & 100 & 1 \\[0.20em]
SN2013bt & $+0.05\pm{0.13}$ & $0.0367$ & $-0.11\pm{0.03}$ & $-2.12\pm{0.14}$ & $6.87^{+0.29}_{-0.34}$ &$-3.92^{+0.33}_{-0.59}$&$-10.8^{+0.5}_{-0.6}$& $10.98^{+0.10}_{-0.10}$ & 51 & 100 & 1 \\[0.20em]
\hline

\caption*{\textbf{Notes:} \\
$\Delta\,m_B^{corr}$ includes a $0.094\,\mathrm{mag}$ residual dispersion.\\[-0.40em] 
Heliocentric redshifts are taken from \cite{childress_2013b}, 
except for LSQ12ekl, LSQ13vy, PTF10wnm PTF10xyt, PTF10zdk, and PTF11mty, \\[-0.40em]
for which heliocentric redshifts were derived from our local H$\alpha$ 
measurements. \\ [-0.4em]
\PY\ is the statistical classification
for a SN~Ia to be young, as given Eq.~\ref{eq:p(delayed)}. \\[-0.40em]
\PM\ is the probability for
the global stellar mass of the SN host galaxy to be higher  % or lower
than $\log(M_*/M_\odot)=10$.\\[-0.40em]
The Refs column provides references for external discoveries, as follows:
%\tablebib*{
(1) \cite{drake_2009} 
(2) \cite{maguire_2012} 
(3) \cite{barone-nugent_2012}
(4) \cite{maguire_2013} \\ [-0.40em]
(5) \cite{weyant_2014}
(6) \cite{maguire_2014}
(7) Boles; Armstrong 
(8) del Olmo, Martinez,Pedraz, Alises; Trondal, Schwartz 
(9) \cite{SDSSII} 
(10) Quimby et al \\ [-0.40em] 
(11) \cite{kelly_2010} 
(12) LOSS
(13) \cite{blondin_2012} 
(14) Ciabattari, Donati, Mazzoni 
(15) Arbour 
(16) Ciabattari et al.
(17) \cite{THU-NAOC}
%}
}

\end{longtable}
%\end{tabularx}

\end{landscape}


==> magdata.tex <==
\begin{landscape}
\begin{longtable}{l|ccccccccccc}

%\centering
\caption{Data for the \nSNe\ SNe~Ia used in this analysis.} \label{tab:lowleveldatalong}\\
%\footnotesize{
%\renewcommand{\arraystretch}{1.3}
%\setlength{\tabcolsep}{3pt}


\hline\hline%\\[-0.8em]

{SN Name} & {SN RA} & {SN Dec} & {host RA} & {host Dec} & {Local $g$} & {Local $i$} &
                                                                  {Global $g$}
  & {Global $i$} & {Note}\\
                & \small{$\mathrm{degree}$} &\small{$\mathrm{degree}$} &
                                                         \small{$\mathrm{degree}$}& \small{$\mathrm{degree}$} &
\small{$\mathrm{mag}$}& \small{$\mathrm{mag}$} & \small{$\mathrm{mag}$} & \small{$\mathrm{mag}$} &\\[0.15em]
\hline\\[-0.8em]

\endfirsthead

\caption{continued.}\\

{SN Name} & {SN RA} & {SN Dec} & {host RA} & {host Dec} & {Local $g$} & {Local $i$} &
                                                                  {Global $g$}
  & {Global $i$} & {Note}\\
                & \small{$\mathrm{degree}$} &\small{$\mathrm{degree}$} &
                                                         \small{$\mathrm{degree}$}& \small{$\mathrm{degree}$} &
\small{$\mathrm{mag}$}& \small{$\mathrm{mag}$} & \small{$\mathrm{mag}$} & \small{$\mathrm{mag}$} &\\[0.15em]
\hline\\[-0.8em]

\endhead

%\hline\\[-0.8em]
\endfoot

\endlastfoot
SNF20050624-000 &+263.6979&-2.3568&+263.6935&-2.3575&$23.97^{+1.15}_{-0.64}$ &$23.48^{+1.17}_{-0.67}$ &$16.23^{+0.01}_{-0.01}$ &$15.25^{+0.01}_{-0.01}$ &a \\[0.20em]
SNF20050728-000 &+14.3730&-22.5872&+14.3734&-22.5874&$20.60^{+0.03}_{-0.03}$ &$20.13^{+0.06}_{-0.05}$ &$17.96^{+0.01}_{-0.01}$ &$17.97^{+0.02}_{-0.02}$ &a \\[0.20em]
SNF20050728-006 &+329.5180&-13.9986&+329.5207&-14.0008&$22.87^{+0.25}_{-0.20}$ &$21.99^{+0.27}_{-0.21}$ &$18.06^{+0.02}_{-0.02}$ &$16.95^{+0.01}_{-0.01}$ &a \\[0.20em]
SNF20050821-007 &+22.6216&+9.2403&+22.6224&+9.2403&$22.13^{+0.08}_{-0.08}$ &$21.55^{+0.11}_{-0.11}$ &$19.19^{+0.02}_{-0.02}$ &$18.66^{+0.03}_{-0.03}$ & \\[0.20em]
SNF20050829-003 &+336.7188&+10.4896&+336.7175&+10.4886&$22.90^{+0.23}_{-0.18}$ &$21.95^{+0.23}_{-0.19}$ &$16.56^{+0.01}_{-0.01}$ &$15.87^{+0.01}_{-0.01}$ & \\[0.20em]
SNF20050927-005 &+39.1590&+8.6426&+39.1593&+8.6425&$19.43^{+0.02}_{-0.02}$ &$18.88^{+0.02}_{-0.02}$ &$16.96^{+0.01}_{-0.01}$ &$16.47^{+0.01}_{-0.01}$ &a \\[0.20em]
SNF20051003-004 &+36.9303&+28.1768&+36.9305&+28.1771&$18.73^{+0.01}_{-0.01}$ &$18.16^{+0.01}_{-0.01}$ &$17.62^{+0.01}_{-0.01}$ &$17.01^{+0.01}_{-0.01}$ &a \\[0.20em]
SNF20060511-014 &+315.1390&-24.6175&+315.1336&-24.6173&$23.26^{+0.44}_{-0.31}$ &$22.24^{+0.39}_{-0.29}$ &$16.45^{+0.01}_{-0.01}$ &$15.57^{+0.01}_{-0.01}$ &a \\[0.20em]
SNF20060512-001 &+213.3541&+17.7833&+213.3538&+17.7830&$19.23^{+0.01}_{-0.01}$ &$18.53^{+0.01}_{-0.01}$ &$17.44^{+0.01}_{-0.01}$ &$16.84^{+0.01}_{-0.01}$ & \\[0.20em]
SNF20060512-002 &+218.3799&+17.0200&+218.3799&+17.0199&$19.01^{+0.01}_{-0.01}$ &$17.63^{+0.01}_{-0.01}$ &$15.98^{+0.01}_{-0.01}$ &$14.86^{+0.01}_{-0.01}$ & \\[0.20em]
SNF20060521-001 &+184.2208&-3.2581&+184.2208&-3.2580&$20.37^{+0.02}_{-0.02}$ &$19.26^{+0.01}_{-0.01}$ &$18.89^{+0.01}_{-0.01}$ &$17.72^{+0.01}_{-0.01}$ & \\[0.20em]
SNF20060521-008 &+191.0160&-5.1028&+191.0125&-5.1095&$23.86^{+0.36}_{-0.27}$ &$22.94^{+0.41}_{-0.29}$ &$15.92^{+0.01}_{-0.01}$ &$14.61^{+0.01}_{-0.01}$ & \\[0.20em]
SNF20060526-003 &+220.7628&-18.8790&+220.7606&-18.8772&$24.11^{+0.39}_{-0.30}$ &$23.79^{+0.90}_{-0.51}$ &$16.08^{+0.01}_{-0.01}$ &$15.47^{+0.01}_{-0.01}$ &a \\[0.20em]
SNF20060530-003 &+244.4678&-0.3336&+244.4666&-0.3326&$21.95^{+0.07}_{-0.06}$ &$21.27^{+0.07}_{-0.07}$ &$17.06^{+0.01}_{-0.01}$ &$16.18^{+0.01}_{-0.01}$ & \\[0.20em]
SNF20060609-002 &+241.1269&+17.4688&+241.1268&+17.4692&$19.08^{+0.01}_{-0.01}$ &$18.16^{+0.01}_{-0.01}$ &$15.31^{+0.01}_{-0.01}$ &$14.47^{+0.01}_{-0.01}$ & \\[0.20em]
SNF20060618-014 &+221.9862&+2.8719&+221.9859&+2.8719&$22.15^{+0.08}_{-0.07}$ &$21.43^{+0.09}_{-0.08}$ &$20.01^{+0.03}_{-0.03}$ &$19.38^{+0.04}_{-0.03}$ & \\[0.20em]
SNF20060621-012 &+306.6753&-12.2080&+306.6751&-12.2080&$21.70^{+0.05}_{-0.05}$ &$20.82^{+0.06}_{-0.05}$ &$18.90^{+0.02}_{-0.02}$ &$18.28^{+0.03}_{-0.03}$ & \\[0.20em]
SNF20060621-015 &+318.8834&-13.4015&+318.8827&-13.4009&$21.75^{+0.06}_{-0.05}$ &$21.50^{+0.11}_{-0.10}$ &$18.03^{+0.01}_{-0.01}$ &$17.60^{+0.01}_{-0.01}$ & \\[0.20em]
SNF20060624-019 &+264.6874&+4.1974&+264.6880&+4.1970&$21.79^{+0.07}_{-0.07}$ &$20.82^{+0.05}_{-0.05}$ &$17.84^{+0.01}_{-0.01}$ &$16.78^{+0.01}_{-0.01}$ & \\[0.20em]
SNF20060907-000 &+315.2991&+21.4005&+315.2992&+21.4003&$19.79^{+0.01}_{-0.01}$ &$18.83^{+0.02}_{-0.02}$ &$17.69^{+0.01}_{-0.01}$ &$17.02^{+0.01}_{-0.01}$ &a \\[0.20em]
SNF20060912-000 &+13.1864&-8.2854&+13.1880&-8.2866&$22.34^{+0.10}_{-0.09}$ &$21.61^{+0.10}_{-0.09}$ &$16.64^{+0.01}_{-0.01}$ &$15.60^{+0.01}_{-0.01}$ & \\[0.20em]
SNF20060912-004 &+24.1165&-5.6718&+24.1151&-5.6727&$23.04^{+0.15}_{-0.13}$ &$22.34^{+0.15}_{-0.13}$ &$16.78^{+0.01}_{-0.01}$ &$15.66^{+0.01}_{-0.01}$ & \\[0.20em]
SNF20060916-002 &+12.6475&+4.7940&+12.6474&+4.7946&$22.80^{+0.10}_{-0.09}$ &$22.15^{+0.12}_{-0.11}$ &$19.52^{+0.03}_{-0.02}$ &$19.01^{+0.03}_{-0.03}$ & \\[0.20em]
SNF20061011-005 &+41.6676&-1.8042&+41.6682&-1.8052&$19.55^{+0.02}_{-0.02}$ &$19.24^{+0.03}_{-0.03}$ &$17.17^{+0.01}_{-0.01}$ &$16.89^{+0.03}_{-0.02}$ & \\[0.20em]
SNF20061020-000 &+10.2704&+6.7941&+10.2717&+6.7956&$20.72^{+0.03}_{-0.03}$ &$19.71^{+0.02}_{-0.02}$ &$16.78^{+0.01}_{-0.01}$ &$15.62^{+0.01}_{-0.01}$ & \\[0.20em]
SNF20061021-003 &+9.0572&+7.1689&+9.0564&+7.1668&$22.29^{+0.07}_{-0.07}$ &$21.12^{+0.06}_{-0.05}$ &$16.02^{+0.01}_{-0.01}$ &$14.74^{+0.01}_{-0.01}$ & \\[0.20em]
SNF20061022-005 &+10.1580&-8.8818&+10.1585&-8.8814&$22.15^{+0.06}_{-0.06}$ &$20.94^{+0.05}_{-0.05}$ &$17.83^{+0.01}_{-0.01}$ &$16.73^{+0.01}_{-0.01}$ & \\[0.20em]
SNF20061022-014 &+351.7725&+4.4261&+351.7717&+4.4259&$20.12^{+0.02}_{-0.02}$ &$18.89^{+0.01}_{-0.01}$ &$16.17^{+0.01}_{-0.01}$ &$14.83^{+0.01}_{-0.01}$ & \\[0.20em]
SNF20061024-000 &+30.9883&-5.8723&+30.9880&-5.8747&$22.79^{+0.12}_{-0.11}$ &$21.53^{+0.09}_{-0.08}$ &$16.55^{+0.01}_{-0.01}$ &$15.39^{+0.01}_{-0.01}$ & \\[0.20em]
SNF20061030-010 &+49.5840&-2.3134&+49.5842&-2.3136&$18.12^{+0.01}_{-0.01}$ &$17.51^{+0.01}_{-0.01}$ &$16.53^{+0.01}_{-0.01}$ &$15.83^{+0.01}_{-0.01}$ &a \\[0.20em]
SNF20061111-002 &+346.8280&-13.5188&+346.8282&-13.5183&$23.70^{+0.47}_{-0.34}$ &$23.40^{+0.96}_{-0.55}$ &$19.62^{+0.03}_{-0.03}$ &$19.11^{+0.04}_{-0.04}$ &a \\[0.20em]
SNF20070330-024 &+204.5585&-20.3460&+204.5568&-20.3468&$20.47^{+0.02}_{-0.02}$ &$19.29^{+0.02}_{-0.02}$ &$14.89^{+0.01}_{-0.01}$ &$13.74^{+0.01}_{-0.01}$ &a \\[0.20em]
SNF20070331-014 &+161.0665&+34.9471&+161.0725&+34.9447&$25.86^{+1.23}_{-0.76}$ &$24.26^{+0.87}_{-0.55}$ &$15.69^{+0.01}_{-0.01}$ &$14.58^{+0.01}_{-0.01}$ & \\[0.20em]
SNF20070403-000 &+161.2368&+23.2637&+161.2360&+23.2620&$21.92^{+0.05}_{-0.05}$ &$21.10^{+0.06}_{-0.06}$ &$17.95^{+0.01}_{-0.01}$ &$16.83^{+0.01}_{-0.01}$ & \\[0.20em]
SNF20070424-003 &+224.4763&+18.6047&+224.4770&+18.6058&$23.53^{+0.18}_{-0.15}$ &$22.99^{+0.29}_{-0.23}$ &$18.59^{+0.01}_{-0.01}$ &$17.91^{+0.01}_{-0.01}$ & \\[0.20em]
SNF20070427-001 &+164.0143&+28.1443&+164.0156&+28.1438&$23.81^{+0.19}_{-0.17}$ &$22.94^{+0.23}_{-0.19}$ &$17.74^{+0.01}_{-0.01}$ &$16.50^{+0.01}_{-0.01}$ & \\[0.20em]
SNF20070429-000 &+212.5158&+33.1687&+212.5152&+33.1675&$21.71^{+0.05}_{-0.04}$ &$21.31^{+0.06}_{-0.06}$ &$16.80^{+0.01}_{-0.01}$ &$16.15^{+0.01}_{-0.01}$ & \\[0.20em]
SNF20070506-006 &+227.3969&+4.8761&+227.3940&+4.8748&$21.24^{+0.05}_{-0.05}$ &$20.91^{+0.07}_{-0.07}$ &$15.74^{+0.01}_{-0.01}$ &$15.19^{+0.01}_{-0.01}$ & \\[0.20em]
SNF20070531-011 &+220.7150&+8.7607&+220.7142&+8.7589&$20.15^{+0.02}_{-0.02}$ &$19.21^{+0.02}_{-0.02}$ &$14.95^{+0.01}_{-0.01}$ &$13.83^{+0.01}_{-0.01}$ & \\[0.20em]
SNF20070630-006 &+353.8653&+19.2230&+353.8647&+19.2238&$22.55^{+0.10}_{-0.09}$ &$21.94^{+0.14}_{-0.12}$ &$17.99^{+0.01}_{-0.01}$ &$17.38^{+0.02}_{-0.02}$ & \\[0.20em]
SNF20070701-005 &+351.2867&-9.9787&+351.2858&-9.9797&$21.83^{+0.05}_{-0.05}$ &$20.92^{+0.05}_{-0.05}$ &$16.21^{+0.01}_{-0.01}$ &$15.22^{+0.01}_{-0.01}$ & \\[0.20em]
SNF20070712-000 &+266.5480&+55.2652&+266.5465&+55.2667&$20.06^{+0.02}_{-0.02}$ &$19.48^{+0.02}_{-0.02}$ &$15.68^{+0.01}_{-0.01}$ &$14.94^{+0.01}_{-0.01}$ & \\[0.20em]
SNF20070712-003 &+250.6676&+50.5975&+250.6681&+50.5974&$23.26^{+0.17}_{-0.15}$ &$22.64^{+0.20}_{-0.17}$ &$21.67^{+0.08}_{-0.07}$ &$21.24^{+0.13}_{-0.11}$ & \\[0.20em]
SNF20070714-007 &+236.6631&+3.4958&+236.6650&+3.4936&$20.67^{+0.03}_{-0.03}$ &$19.94^{+0.03}_{-0.03}$ &$16.47^{+0.01}_{-0.01}$ &$15.28^{+0.01}_{-0.01}$ & \\[0.20em]
SNF20070725-001 &+316.2582&+8.2715&+316.2577&+8.2733&$23.67^{+0.32}_{-0.24}$ &$23.52^{+0.69}_{-0.43}$ &$18.82^{+0.02}_{-0.02}$ &$18.35^{+0.03}_{-0.03}$ & \\[0.20em]
SNF20070727-016 &+243.6240&+56.0681&+243.6254&+56.0698&$24.14^{+0.34}_{-0.27}$ &$23.03^{+0.31}_{-0.25}$ &$16.80^{+0.01}_{-0.01}$ &$15.57^{+0.01}_{-0.01}$ & \\[0.20em]
SNF20070802-000 &+243.7161&+56.3949&+243.7154&+56.3991&$23.57^{+0.24}_{-0.20}$ &$22.52^{+0.19}_{-0.16}$ &$15.59^{+0.01}_{-0.01}$ &$14.29^{+0.01}_{-0.01}$ & \\[0.20em]
SNF20070806-026 &+328.4684&+4.4952&+328.4696&+4.4985&$22.89^{+0.19}_{-0.16}$ &$21.82^{+0.16}_{-0.14}$ &$15.87^{+0.01}_{-0.01}$ &$14.60^{+0.01}_{-0.01}$ & \\[0.20em]
SNF20070818-001 &+17.7285&-6.4539&+17.7305&-6.4525&$23.66^{+0.40}_{-0.29}$ &$22.88^{+0.41}_{-0.28}$ &$17.43^{+0.02}_{-0.02}$ &$16.50^{+0.02}_{-0.01}$ & \\[0.20em]
SNF20070820-000 &+340.9286&+24.3656&+340.9292&+24.3662&$21.28^{+0.04}_{-0.04}$ &$20.42^{+0.04}_{-0.04}$ &$18.18^{+0.01}_{-0.01}$ &$17.02^{+0.01}_{-0.01}$ & \\[0.20em]
SNF20070831-015 &+337.8565&+10.7948&+337.8570&+10.7950&$21.08^{+0.03}_{-0.03}$ &$20.27^{+0.03}_{-0.03}$ &$17.26^{+0.01}_{-0.01}$ &$16.51^{+0.01}_{-0.01}$ & \\[0.20em]
SNF20070902-018 &+20.2891&-4.2377&+20.2889&-4.2365&$21.66^{+0.04}_{-0.04}$ &$20.62^{+0.04}_{-0.03}$ &$17.68^{+0.01}_{-0.01}$ &$16.54^{+0.01}_{-0.01}$ & \\[0.20em]
SNF20070902-021 &+7.5029&+33.2927&+7.5031&+33.2923&$22.53^{+0.13}_{-0.12}$ &$21.69^{+0.15}_{-0.14}$ &$18.76^{+0.02}_{-0.02}$ &$18.02^{+0.02}_{-0.02}$ &a \\[0.20em]
SNF20071003-004 &+41.2037&-16.3249&+41.2030&-16.3251&$24.04^{+0.28}_{-0.22}$ &$23.35^{+0.40}_{-0.29}$ &$18.82^{+0.02}_{-0.02}$ &$18.42^{+0.03}_{-0.03}$ & \\[0.20em]
SNF20071003-016 &+36.8590&+9.7502&+36.8591&+9.7498&$21.21^{+0.03}_{-0.04}$ &$20.25^{+0.05}_{-0.05}$ &$19.21^{+0.02}_{-0.02}$ &$18.59^{+0.03}_{-0.03}$ &a \\[0.20em]
SNF20071015-000 &+346.3934&+9.1243&+346.3927&+9.1211&$20.22^{+0.02}_{-0.02}$ &$19.46^{+0.02}_{-0.02}$ &$15.19^{+0.01}_{-0.01}$ &$14.15^{+0.01}_{-0.01}$ & \\[0.20em]
SNF20071021-000 &+3.7493&+16.3350&+3.7505&+16.3333&$20.16^{+0.03}_{-0.03}$ &$19.66^{+0.03}_{-0.03}$ &$15.99^{+0.01}_{-0.01}$ &$15.29^{+0.01}_{-0.01}$ & \\[0.20em]
SNF20071108-021 &+121.5263&+30.5466&+121.5255&+30.5461&$23.21^{+0.13}_{-0.12}$ &$22.48^{+0.18}_{-0.15}$ &$18.69^{+0.02}_{-0.02}$ &$18.36^{+0.03}_{-0.03}$ & \\[0.20em]
SNF20080507-000 &+243.7789&+50.2785&+243.7787&+50.2784&$20.13^{+0.02}_{-0.02}$ &$19.21^{+0.01}_{-0.01}$ &$17.12^{+0.01}_{-0.01}$ &$16.19^{+0.01}_{-0.01}$ & \\[0.20em]
SNF20080510-001 &+224.0555&+18.8539&+224.0553&+18.8540&$25.33^{+1.07}_{-0.64}$ &$24.00^{+0.71}_{-0.43}$ &$23.05^{+1.60}_{-0.70}$ &$20.92^{+1.20}_{-0.90}$ & \\[0.20em]
SNF20080512-008 &+255.8964&+31.3533&+255.8968&+31.3533&$25.94^{+1.22}_{-0.72}$ &$24.34^{+0.82}_{-0.50}$ &$22.29^{+0.19}_{-0.16}$ &$21.86^{+0.29}_{-0.23}$ & \\[0.20em]
SNF20080512-010 &+242.7681&+52.4522&+242.7670&+52.4503&$21.46^{+0.04}_{-0.04}$ &$20.17^{+0.02}_{-0.02}$ &$14.47^{+0.01}_{-0.01}$ &$13.18^{+0.01}_{-0.01}$ & \\[0.20em]
SNF20080514-002 &+202.3034&+11.2724&+202.3068&+11.2758&$19.40^{+0.01}_{-0.01}$ &$18.28^{+0.01}_{-0.01}$ &$14.43^{+0.01}_{-0.01}$ &$13.25^{+0.01}_{-0.01}$ & \\[0.20em]
SNF20080516-000 &+170.6238&+56.4074&+170.6239&+56.4074&$23.10^{+0.11}_{-0.11}$ &$22.49^{+0.16}_{-0.13}$ &$19.73^{+0.04}_{-0.04}$ &$19.34^{+0.09}_{-0.08}$ & \\[0.20em]
SNF20080516-022 &+224.8665&+58.0027&+224.8627&+58.0017&$26.07^{+1.24}_{-0.76}$ &$24.05^{+0.69}_{-0.47}$ &$17.52^{+0.01}_{-0.01}$ &$16.25^{+0.01}_{-0.01}$ & \\[0.20em]
SNF20080522-011 &+229.9955&+4.9047&+229.9953&+4.9047&$20.06^{+0.02}_{-0.02}$ &$19.63^{+0.02}_{-0.02}$ &$18.50^{+0.01}_{-0.01}$ &$18.16^{+0.02}_{-0.02}$ & \\[0.20em]
SNF20080531-000 &+244.2487&+19.1172&+244.2503&+19.1181&$20.33^{+0.02}_{-0.02}$ &$19.98^{+0.03}_{-0.03}$ &$15.81^{+0.01}_{-0.01}$ &$15.15^{+0.01}_{-0.01}$ & \\[0.20em]
SNF20080610-000 &+228.4540&+1.8616&+228.4546&+1.8617&$23.62^{+0.20}_{-0.17}$ &$22.90^{+0.22}_{-0.18}$ &$19.66^{+0.03}_{-0.03}$ &$19.23^{+0.04}_{-0.04}$ & \\[0.20em]
SNF20080612-003 &+243.8682&+19.2266&+243.8692&+19.2261&$20.38^{+0.02}_{-0.02}$ &$19.31^{+0.02}_{-0.02}$ &$16.97^{+0.01}_{-0.01}$ &$15.88^{+0.01}_{-0.01}$ & \\[0.20em]
SNF20080614-010 &+216.7210&+23.9353&+216.7209&+23.9366&$23.31^{+0.15}_{-0.13}$ &$22.17^{+0.11}_{-0.10}$ &$17.65^{+0.01}_{-0.01}$ &$16.39^{+0.01}_{-0.01}$ & \\[0.20em]
SNF20080620-000 &+242.5728&+22.7258&+242.5727&+22.7258&$19.19^{+0.01}_{-0.01}$ &$18.54^{+0.01}_{-0.01}$ &$18.00^{+0.01}_{-0.01}$ &$17.39^{+0.01}_{-0.01}$ & \\[0.20em]
SNF20080623-001 &+272.9164&+50.1810&+272.9152&+50.1826&$23.97^{+0.44}_{-0.31}$ &$23.22^{+0.83}_{-0.49}$ &$18.85^{+0.01}_{-0.01}$ &$18.32^{+0.02}_{-0.02}$ &a \\[0.20em]
SNF20080717-000 &+1.7262&+24.9979&+1.7274&+24.9981&$21.04^{+0.03}_{-0.03}$ &$19.88^{+0.02}_{-0.02}$ &$17.21^{+0.01}_{-0.01}$ &$16.08^{+0.01}_{-0.01}$ & \\[0.20em]
SNF20080725-004 &+354.3413&+19.9314&+354.3419&+19.9315&$20.54^{+0.02}_{-0.02}$ &$19.78^{+0.03}_{-0.03}$ &$18.03^{+0.01}_{-0.01}$ &$17.03^{+0.01}_{-0.01}$ & \\[0.20em]
SNF20080731-000 &+266.0131&+33.0410&+266.0137&+33.0405&$23.22^{+0.13}_{-0.12}$ &$22.02^{+0.18}_{-0.16}$ &$18.82^{+0.01}_{-0.01}$ &$17.66^{+0.02}_{-0.02}$ &a \\[0.20em]
SNF20080802-006 &+23.4032&+28.1333&+23.4046&+28.1327&$23.06^{+0.16}_{-0.14}$ &$22.08^{+0.14}_{-0.12}$ &$17.16^{+0.01}_{-0.01}$ &$15.92^{+0.01}_{-0.01}$ & \\[0.20em]
SNF20080803-000 &+255.0300&+23.1324&+255.0287&+23.1315&$21.38^{+0.04}_{-0.04}$ &$20.59^{+0.04}_{-0.04}$ &$16.32^{+0.01}_{-0.01}$ &$15.23^{+0.01}_{-0.01}$ & \\[0.20em]
SNF20080806-002 &+259.7265&+45.5437&+259.7274&+45.5433&$20.59^{+0.02}_{-0.02}$ &$19.77^{+0.02}_{-0.02}$ &$17.04^{+0.01}_{-0.01}$ &$16.02^{+0.01}_{-0.01}$ & \\[0.20em]
SNF20080810-001 &+264.9032&+37.8688&+264.9072&+37.8680&$22.95^{+0.15}_{-0.14}$ &$22.09^{+0.25}_{-0.20}$ &$15.54^{+0.01}_{-0.01}$ &$14.63^{+0.01}_{-0.01}$ &a \\[0.20em]
SNF20080815-017 &+337.5721&+24.9932&+337.5700&+24.9927&$22.51^{+0.08}_{-0.08}$ &$21.29^{+0.08}_{-0.08}$ &$15.85^{+0.01}_{-0.01}$ &$14.60^{+0.01}_{-0.01}$ & \\[0.20em]
SNF20080821-000 &+306.0830&+6.1745&+306.0841&+6.1744&$20.92^{+0.03}_{-0.03}$ &$20.09^{+0.02}_{-0.02}$ &$16.86^{+0.01}_{-0.01}$ &$15.91^{+0.01}_{-0.01}$ & \\[0.20em]
SNF20080822-005 &+357.3428&+19.2073&+357.3412&+19.2066&$22.36^{+0.08}_{-0.07}$ &$21.47^{+0.09}_{-0.09}$ &$16.27^{+0.01}_{-0.01}$ &$15.13^{+0.01}_{-0.01}$ & \\[0.20em]
SNF20080825-010 &+24.4200&-13.3121&+24.4202&-13.3146&$21.16^{+0.06}_{-0.05}$ &$19.97^{+0.05}_{-0.04}$ &$14.90^{+0.01}_{-0.01}$ &$13.80^{+0.01}_{-0.01}$ &a \\[0.20em]
SNF20080908-000 &+341.8026&-19.5789&+341.8024&-19.5793&$22.13^{+0.11}_{-0.10}$ &$21.87^{+0.20}_{-0.18}$ &$19.96^{+0.04}_{-0.04}$ &$19.52^{+0.06}_{-0.06}$ & \\[0.20em]
SNF20080909-030 &+330.4544&+13.0553&+330.4559&+13.0549&$21.78^{+0.09}_{-0.09}$ &$21.76^{+0.21}_{-0.18}$ &$19.55^{+0.03}_{-0.03}$ &$18.06^{+0.02}_{-0.02}$ & \\[0.20em]
SNF20080913-031 &+32.8916&+23.8804&+32.8846&+23.8853&$24.20^{+0.60}_{-0.38}$ &$23.07^{+0.47}_{-0.33}$ &$16.88^{+0.01}_{-0.01}$ &$15.68^{+0.01}_{-0.01}$ & \\[0.20em]
SNF20080914-001 &+74.3642&-0.0690&+74.3624&-0.0707&$19.76^{+0.02}_{-0.02}$ &$18.69^{+0.02}_{-0.02}$ &$16.22^{+0.01}_{-0.01}$ &$15.04^{+0.01}_{-0.01}$ & \\[0.20em]
SNF20080918-000 &+353.3290&+25.2141&+353.3301&+25.2127&$22.08^{+0.09}_{-0.09}$ &$21.66^{+0.14}_{-0.13}$ &$17.25^{+0.01}_{-0.01}$ &$16.33^{+0.01}_{-0.01}$ &a \\[0.20em]
SNF20080919-001 &+16.6864&-11.1264&+16.6865&-11.1258&$21.65^{+0.19}_{-0.16}$ &$20.67^{+0.09}_{-0.08}$ &$19.28^{+0.08}_{-0.07}$ &$19.03^{+0.04}_{-0.04}$ &a \\[0.20em]
SNF20080919-002 &+36.3383&-8.6498&+36.3371&-8.6506&$22.30^{+0.08}_{-0.07}$ &$21.53^{+0.09}_{-0.08}$ &$17.12^{+0.01}_{-0.01}$ &$16.35^{+0.01}_{-0.01}$ & \\[0.20em]
SNF20080920-000 &+35.1413&+4.4546&+35.1417&+4.4550&$19.94^{+0.02}_{-0.02}$ &$19.38^{+0.02}_{-0.02}$ &$16.34^{+0.01}_{-0.01}$ &$15.87^{+0.01}_{-0.01}$ &a \\[0.20em]
SNF20080926-009 &+332.0932&-10.9725&+332.0944&-10.9718&$24.13^{+0.67}_{-0.44}$ &$23.29^{+0.80}_{-0.48}$ &$18.97^{+0.02}_{-0.02}$ &$18.49^{+0.03}_{-0.03}$ &a \\[0.20em]
CSS120424\_01 &+210.5677&-11.3524&+210.5627&-11.3496&$22.72^{+0.19}_{-0.16}$ &$22.57^{+0.39}_{-0.30}$ &$15.51^{+0.01}_{-0.01}$ &$14.81^{+0.01}_{-0.01}$ & \\[0.20em]
CSS130502\_01 &+175.0419&+30.0294&+175.0460&+30.0290&$23.13^{+0.22}_{-0.18}$ &$22.35^{+0.29}_{-0.23}$ &$17.27^{+0.01}_{-0.01}$ &$16.76^{+0.01}_{-0.01}$ & \\[0.20em]
LSQ12ekl &+347.8560&-1.8651&+347.8565&-1.8652&$23.56^{+0.21}_{-0.17}$ &$22.95^{+0.34}_{-0.25}$ &$18.68^{+0.02}_{-0.02}$ &$17.96^{+0.03}_{-0.02}$ & \\[0.20em]
LSQ12fmx &+48.2172&-0.2036&+48.2206&-0.2067&$25.51^{+1.16}_{-0.71}$ &$24.07^{+0.87}_{-0.53}$ &$16.74^{+0.01}_{-0.01}$ &$15.98^{+0.01}_{-0.01}$ & \\[0.20em]
LSQ13vy &+241.7327&+3.0042&+241.7318&+3.0012&$21.58^{+0.06}_{-0.06}$ &$20.92^{+0.07}_{-0.06}$ &$16.02^{+0.01}_{-0.01}$ &$15.01^{+0.01}_{-0.01}$ & \\[0.20em]
PTF09dlc &+326.6254&+6.4192&+326.6251&+6.4187&$22.97^{+0.13}_{-0.12}$ &$22.87^{+0.28}_{-0.22}$ &$19.78^{+0.03}_{-0.03}$ &$19.30^{+0.04}_{-0.04}$ & \\[0.20em]
PTF09dnl &+260.9242&+30.4971&+260.9237&+30.4975&$20.47^{+0.03}_{-0.03}$ &$19.91^{+0.04}_{-0.04}$ &$19.45^{+0.03}_{-0.03}$ &$18.99^{+0.06}_{-0.05}$ & \\[0.20em]
PTF09dnp &+229.8518&+49.4990&+229.8556&+49.5014&$22.43^{+0.11}_{-0.10}$ &$21.59^{+0.13}_{-0.11}$ &$15.51^{+0.01}_{-0.01}$ &$14.33^{+0.01}_{-0.01}$ & \\[0.20em]
PTF09foz &+10.5488&-9.8812&+10.5496&-9.8819&$21.00^{+0.03}_{-0.03}$ &$19.93^{+0.03}_{-0.03}$ &$16.37^{+0.01}_{-0.01}$ &$15.31^{+0.01}_{-0.01}$ & \\[0.20em]
PTF10hmv &+182.8886&+47.2749&+182.8888&+47.2746&$20.76^{+0.03}_{-0.03}$ &$20.04^{+0.03}_{-0.03}$ &$19.59^{+0.02}_{-0.02}$ &$19.02^{+0.02}_{-0.02}$ & \\[0.20em]
PTF10mwb &+259.4579&+40.8811&+259.4585&+40.8813&$20.92^{+0.04}_{-0.03}$ &$20.10^{+0.04}_{-0.04}$ &$18.07^{+0.02}_{-0.02}$ &$17.35^{+0.02}_{-0.02}$ & \\[0.20em]
PTF10qjl &+249.9975&+12.1072&+249.9968&+12.1074&$22.19^{+0.07}_{-0.07}$ &$21.90^{+0.13}_{-0.12}$ &$18.82^{+0.01}_{-0.01}$ &$18.51^{+0.02}_{-0.01}$ & \\[0.20em]
PTF10qjq &+256.8017&+35.5098&+256.8015&+35.5099&$17.34^{+0.01}_{-0.01}$ &$16.84^{+0.01}_{-0.01}$ &$15.75^{+0.01}_{-0.01}$ &$15.12^{+0.01}_{-0.01}$ & \\[0.20em]
PTF10tce &+349.7927&+9.1984&+349.7906&+9.1960&$22.38^{+0.11}_{-0.10}$ &$21.49^{+0.10}_{-0.10}$ &$16.03^{+0.01}_{-0.01}$ &$15.21^{+0.01}_{-0.01}$ & \\[0.20em]
PTF10wnm &+5.5150&+27.0406&+5.5153&+27.0393&$21.83^{+0.04}_{-0.04}$ &$21.12^{+0.06}_{-0.05}$ &$16.85^{+0.01}_{-0.01}$ &$16.08^{+0.01}_{-0.01}$ & \\[0.20em]
PTF10wof &+353.1745&+15.3588&+353.1726&+15.3588&$21.97^{+0.07}_{-0.06}$ &$21.33^{+0.07}_{-0.07}$ &$17.56^{+0.01}_{-0.01}$ &$16.82^{+0.01}_{-0.01}$ & \\[0.20em]
PTF10xyt &+349.7601&+13.7906&+349.7601&+13.7906&$20.07^{+0.02}_{-0.02}$ &$19.21^{+0.01}_{-0.01}$ &$18.51^{+0.01}_{-0.01}$ &$17.75^{+0.01}_{-0.01}$ & \\[0.20em]
PTF10zdk &+33.5306&+23.6307&+33.5307&+23.6303&$18.48^{+0.01}_{-0.01}$ &$18.20^{+0.01}_{-0.01}$ &$16.07^{+0.01}_{-0.01}$ &$15.84^{+0.01}_{-0.01}$ & \\[0.20em]
PTF11bnx &+247.5805&+21.0853&+247.5823&+21.0854&$21.73^{+0.05}_{-0.04}$ &$21.50^{+0.08}_{-0.08}$ &$17.30^{+0.01}_{-0.01}$ &$16.88^{+0.02}_{-0.02}$ & \\[0.20em]
PTF11cao &+244.6998&+25.1879&+244.6986&+25.1891&$21.24^{+0.04}_{-0.04}$ &$20.63^{+0.05}_{-0.05}$ &$16.99^{+0.01}_{-0.01}$ &$16.32^{+0.01}_{-0.01}$ & \\[0.20em]
PTF11mty &+323.5217&+10.4235&+323.5217&+10.4235&$20.23^{+0.01}_{-0.01}$ &$19.35^{+0.01}_{-0.01}$ &$18.67^{+0.01}_{-0.01}$ &$17.73^{+0.01}_{-0.01}$ & \\[0.20em]
PTF11pbp &+351.9812&+8.7792&+351.9863&+8.7790&$20.64^{+0.04}_{-0.04}$ &$19.76^{+0.04}_{-0.03}$ &$13.49^{+0.01}_{-0.01}$ &$12.69^{+0.01}_{-0.01}$ & \\[0.20em]
PTF12dxm &+208.3604&+43.9135&+208.3659&+43.9126&$24.29^{+0.47}_{-0.33}$ &$22.66^{+0.21}_{-0.19}$ &$15.63^{+0.01}_{-0.01}$ &$14.40^{+0.01}_{-0.01}$ & \\[0.20em]
PTF12iiq &+42.5323&-0.2655&+42.5328&-0.2670&$19.71^{+0.02}_{-0.02}$ &$18.57^{+0.01}_{-0.01}$ &$14.97^{+0.01}_{-0.01}$ &$13.81^{+0.01}_{-0.01}$ & \\[0.20em]
SN2004ef &+340.5417&+19.9946&+340.5439&+19.9969&$20.22^{+0.02}_{-0.02}$ &$19.16^{+0.02}_{-0.02}$ &$14.16^{+0.01}_{-0.01}$ &$13.04^{+0.01}_{-0.01}$ & \\[0.20em]
SN2004gc &+80.4581&+6.6760&+80.4576&+6.6768&$18.29^{+0.01}_{-0.01}$ &$17.40^{+0.01}_{-0.01}$ &$15.82^{+0.01}_{-0.01}$ &$14.86^{+0.01}_{-0.01}$ &a \\[0.20em]
SN2005hc &+29.1998&-0.2137&+29.2021&-0.2126&$21.46^{+0.05}_{-0.04}$ &$20.48^{+0.04}_{-0.04}$ &$15.76^{+0.01}_{-0.01}$ &$14.63^{+0.01}_{-0.01}$ & \\[0.20em]
SN2005hj &+21.7011&-1.2380&+21.7019&-1.2381&$21.46^{+0.05}_{-0.04}$ &$20.48^{+0.04}_{-0.03}$ &$18.80^{+0.02}_{-0.02}$ &$17.76^{+0.01}_{-0.01}$ & \\[0.20em]
SN2005ir &+19.1823&+0.7946&+19.1828&+0.7936&$21.33^{+0.03}_{-0.03}$ &$20.70^{+0.04}_{-0.04}$ &$17.33^{+0.01}_{-0.01}$ &$16.45^{+0.01}_{-0.01}$ & \\[0.20em]
SN2006cj &+194.8518&+28.3477&+194.8505&+28.3472&$22.20^{+0.05}_{-0.05}$ &$21.50^{+0.07}_{-0.07}$ &$17.04^{+0.01}_{-0.01}$ &$15.84^{+0.01}_{-0.01}$ & \\[0.20em]
SN2006dm &+355.4493&-3.6690&+355.4472&-3.6673&$20.45^{+0.05}_{-0.04}$ &$19.30^{+0.03}_{-0.03}$ &$14.53^{+0.01}_{-0.01}$ &$12.83^{+0.01}_{-0.01}$ & \\[0.20em]
SN2006do &+353.0128&-27.7255&+353.0141&-27.7261&$18.92^{+0.01}_{-0.01}$ &$17.71^{+0.01}_{-0.01}$ &$14.25^{+0.01}_{-0.01}$ &$13.20^{+0.01}_{-0.01}$ &a \\[0.20em]
SN2006ob &+27.9505&+0.2634&+27.9521&+0.2638&$21.28^{+0.03}_{-0.03}$ &$20.06^{+0.03}_{-0.03}$ &$15.10^{+0.01}_{-0.01}$ &$13.82^{+0.01}_{-0.01}$ & \\[0.20em]
SN2007bc &+169.8107&+20.8090&+169.8192&+20.8135&$21.17^{+0.08}_{-0.07}$ &$20.19^{+0.06}_{-0.06}$ &$13.77^{+0.01}_{-0.01}$ &$12.56^{+0.01}_{-0.01}$ & \\[0.20em]
SN2007bd &+127.8887&-1.1994&+127.8870&-1.1978&$19.74^{+0.02}_{-0.02}$ &$18.74^{+0.01}_{-0.01}$ &$14.48^{+0.01}_{-0.01}$ &$13.29^{+0.01}_{-0.01}$ & \\[0.20em]
SN2007cq &+333.6685&+5.0803&+333.6696&+5.0786&$19.71^{+0.02}_{-0.02}$ &$19.11^{+0.03}_{-0.03}$ &$15.75^{+0.01}_{-0.01}$ &$15.03^{+0.01}_{-0.01}$ & \\[0.20em]
SN2007kk &+55.5969&+39.2418&+55.6002&+39.2445&$20.76^{+0.04}_{-0.04}$ &$19.88^{+0.03}_{-0.03}$ &$13.77^{+0.01}_{-0.01}$ &$12.73^{+0.01}_{-0.01}$ & \\[0.20em]
SN2007nq &+14.3899&-1.3886&+14.3954&-1.3910&$22.40^{+0.11}_{-0.10}$ &$21.30^{+0.10}_{-0.09}$ &$14.00^{+0.01}_{-0.01}$ &$12.77^{+0.01}_{-0.01}$ & \\[0.20em]
SN2009hi &+350.9844&+16.7749&+350.9893&+16.7772&$21.58^{+0.06}_{-0.06}$ &$20.34^{+0.04}_{-0.04}$ &$13.45^{+0.01}_{-0.01}$ &$12.14^{+0.01}_{-0.01}$ & \\[0.20em]
SN2010dt &+250.8111&+32.6751&+250.8051&+32.6779&$23.26^{+0.17}_{-0.16}$ &$22.65^{+0.27}_{-0.23}$ &$15.75^{+0.01}_{-0.01}$ &$14.89^{+0.01}_{-0.01}$ & \\[0.20em]
SN2010ex &+345.0454&+26.0992&+345.0450&+26.0965&$20.02^{+0.02}_{-0.02}$ &$19.37^{+0.03}_{-0.03}$ &$15.29^{+0.01}_{-0.01}$ &$14.65^{+0.01}_{-0.01}$ & \\[0.20em]
SN2011bc &+181.1372&+20.2032&+181.1355&+20.2049&$18.46^{+0.01}_{-0.01}$ &$17.53^{+0.01}_{-0.01}$ &$13.72^{+0.01}_{-0.01}$ &$12.62^{+0.01}_{-0.01}$ & \\[0.20em]
SN2011be &+140.7192&+21.9877&+140.7211&+21.9752&$20.79^{+0.03}_{-0.03}$ &$20.25^{+0.04}_{-0.03}$ &$14.28^{+0.01}_{-0.01}$ &$13.07^{+0.01}_{-0.01}$ & \\[0.20em]
SN2011ga &+340.1143&+3.1994&+340.1193&+3.1974&$22.87^{+0.19}_{-0.17}$ &$22.28^{+0.27}_{-0.23}$ &$15.40^{+0.01}_{-0.01}$ &$14.37^{+0.01}_{-0.01}$ & \\[0.20em]
SN2011ho &+176.0539&+33.5163&+176.0582&+33.5145&$20.53^{+0.03}_{-0.03}$ &$19.27^{+0.02}_{-0.02}$ &$13.62^{+0.01}_{-0.01}$ &$12.39^{+0.01}_{-0.01}$ & \\[0.20em]
SN2011hv &+349.5690&+0.2620&+349.5653&+0.2612&$19.62^{+0.02}_{-0.01}$ &$18.72^{+0.01}_{-0.01}$ &$14.71^{+0.01}_{-0.01}$ &$13.60^{+0.01}_{-0.01}$ & \\[0.20em]
SN2013be &+189.1153&+11.7578&+189.1133&+11.7593&$22.66^{+0.10}_{-0.09}$ &$21.74^{+0.09}_{-0.08}$ &$16.05^{+0.01}_{-0.01}$ &$14.97^{+0.01}_{-0.01}$ & \\[0.20em]
SN2013bs &+259.3418&+41.0667&+259.3178&+41.0527&$23.92^{+0.68}_{-0.44}$ &$23.07^{+0.75}_{-0.48}$ &$13.92^{+0.01}_{-0.01}$ &$12.72^{+0.01}_{-0.01}$ & \\[0.20em]
SN2013bt &+215.3130&+61.5711&+215.3298&+61.5793&$24.33^{+0.77}_{-0.46}$ &$23.37^{+0.71}_{-0.44}$ &$14.97^{+0.01}_{-0.01}$ &$13.72^{+0.01}_{-0.01}$ & \\[0.20em]


\hline
\caption*{\textbf{Notes:} 
An ``a'' indicates cases where SNIFS host galaxy imaging is used. 
All coordinates are for equinox J2000.
}


\end{longtable}
%\end{tabularx}
%}

\end{landscape}

